Suum Cuique: Studying Bias in Taboo Detection with a Community Perspective

Prior research has discussed and illustrated the need to consider linguistic norms at the community level when studying taboo (hateful/offensive/toxic etc.) language. However, a methodology for doing so, that is firmly founded on community language norms is still largely absent. This can lead both to biases in taboo text classification and limitations in our understanding of the causes of bias. We propose a method to study bias in taboo classification and annotation where a community perspective is front and center. This is accomplished by using special classifiers tuned for each community's language. In essence, these classifiers represent community level language norms. We use these to study bias and find, for example, biases are largest against African Americans (7/10 datasets and all 3 classifiers examined). In contrast to previous papers we also study other communities and find, for example, strong biases against South Asians. In a small scale user study we illustrate our key idea which is that common utterances, i.e., those with high alignment scores with a community (community classifier confidence scores) are unlikely to be regarded taboo. Annotators who are community members contradict taboo classification decisions and annotations in a majority of instances. This paper is a significant step toward reducing false positive taboo decisions that over time harm minority communities.

==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/approach.tex <==
\section{Community Centered Approach for Studying Bias}
%\vspace{-0.5em}


We build community-specific classification models (CLCs) which capture the community's language.
We use these to compute text alignment scores for assessing bias.
A text alignment score is the classifier's confidence in deciding if the text has been generated by a member of the community or not. Higher confidence scores imply greater alignment with the language norm's of the community. 
%for each minority community of interest using representative data.
%These models can be used to obtain likelihood scores for any new text, referred to here as alignment scores.  
%We use these scores to detect bias.% in taboo language classifiers and taboo labeled datasets.


%\vspace{-0.25em}
Our intuition is as follows.
Given moderation and self-regulation in communities we expect taboo utterances to be \textit{infrequent} in a community's discourse.
Such utterances will thus have low alignment scores when classified by a model trained on the community's language.
However, since new topics of interest will also result in low-frequency utterances 
we view low alignment scores with a community model as \emph{necessary} but \emph{insufficient} for an utterance to be considered taboo from that community's perspective.
Crucially, utterances with high alignment scores adhere to the norms and therefore should not be considered taboo. 
Reference classifier models allow us to estimate the extent of alignment with community language norms.

Two points to note. We do not attempt to separate style from topic in the utterances since it is often in their interplay that taboo is decided.  For example, \emph{``happy birthday to a bad bitch''} and \emph{``Fuck off, you are a little bitch.''} have somewhat related styles but different topics.
Our `contextual' community-language classification models estimate scores for full utterances.
Second, while we study race/ethnicity based communities, our approach can be applied to communities defined broadly, using other criteria such as professional communities and  internet subcultures. Specific details for measuring bias are given next.\\
\noindent
\textbf{Measuring bias in taboo classifiers:}
%
We assess the extent of taboo classifier bias against a community by  computing Pearson correlation between the taboo classifier confidence scores and community classifier confidence scores.
We do this with instances that the former classifier declares as taboo.
Ideally, we expect a negative correlation - higher taboo classifier confidence mapping to lower community alignment scores and vice versa.
The extent to which correlations deviate from this expectation reflects the extent to which the classifier does not consider the norms of the community.\\
%
%This is similar to the approach taken in \cite{sap2019risk} in which classifiers are trained on taboo datasets and used to label African American and White datasets. 
%They then look at the false positive rate to find if the classifiers label African Americans at a disproportionate rate. 
%
%Our approach differs slightly as we measure bias in classifiers via correlations between membership scores and classifier confidence values.
%in the opposite direction, it means that the classifier does not agree with the community and will label language as taboo even though the community does not find it taboo.
\noindent
\textbf{Measuring bias in taboo datasets:}
%As in previous work for e.g., \cite{sap2019risk} we expect the propensity to produce taboo utterances (\textit{P(taboo|community))} to be equal across communities for a dataset
%\footnote{Note this does not say how high the propensity only that this is even across communities}.
%There is no reason to think one minority community is likely to be more offensive/hateful than another.
%
Given a dataset, we compute the proportion of taboo labelled texts that are  highly aligned with each community classifier
model.
We expect these proportions to be tending towards zero since high alignment means common utterance and thus within the norms.
A second point to note is that if these proportions are uneven across communities then the bias is more against those with larger proportions.
This is consistent with the theory that all communities engage in similar norms of communication \cite{MILLS20091047}.
%
%The first point captures the idea that the language which a community views as taboo will occur less. 
%
%Thus a LM which knows the community's language should also find a lower percentage of taboo labeled data.  
%
%
%Thus, given a dataset %collection we take each taboo labelled instance and measure its alignment with each minority model.
%we compute for each community the proportion of high alignment instances that have been labeled as taboo.
%
Specifically, we measure the mean and standard deviations (SD) of proportion of aligned comments.
%; proportions that are more than 1 SD away from the mean we regard as indicating uneven proportions.
In sum, if the proportions are not close to zero this indicates bias.
%
Additionally, if the proportions are not even then bias is targeting some communities more than others.
%This signals possible weakness in the dataset; perhaps the underlying data collection or annotation process is faulty. 
%
% Yes
%\textbf{does the below hold still?}


==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/bias.tex <==
\section{Experiments and Results}
%\vspace{-0.5em}
\subsection{Taboo Classifier Bias Assessment}
%\vspace{-0.5em}
%[move to intro if anywhere: -Talk about overall trends in the Bias Datasets, then go specific.
%It has been observed in previous research that bias can exist in annotators \cite{binns2017like,waseem2016you}, training data \cite{bolukbasi2016man, kennedy2020contextualizing}, and classifiers \cite{reichert2020reading}. 

%We use our community-specific language models to assess the extent of bias in offense  classifier decisions.
We test 3 SOTA offensive language classifiers:




%and in \textit{taboo\footnote{hate, offense, and abuse}} annotated datasets.


\noindent \textbf{NULI} \cite{liu-etal-2019-nuli}: A BERT \cite{devlin-etal-2019-bert} based system trained on offensive language (OLID \cite{zampierietal2019OLID}). It was the top-ranked system in OffensEval \cite{zampieri2019semeval}. %For preprocessing, the emojis are converted into English and hashtags are segmented. 

\noindent \textbf{MIDAS} \cite{Mahata2019MIDASAS}: An ensemble of three deep learning models: a BLSTM, a BLSTM fed into a BGRU, and a CNN all three trained on offensive language. This system was the top non-BERT based system at OffensEval. 

\noindent \textbf{Perspective} \cite{Perspective}: An API provided by Google, which when given text, returns a toxicity score. The current model in production uses a CNN trained with fine-tuned GloVe word embeddings. 


We trained MIDAS and NULI on the OLID training data which is consistent with their training for OffensEval.
Our implementations perform within 1\% of the published results. 
We then applied the classifiers to the validation datasets listed in Table \ref{tab:communities}.
Correlations between classifier confidence (for Perspective we use its toxicity score) and language model alignment scores were analyzed.


\subsection{Taboo Classifier Bias Results}
%\vspace{-0.5em}
\noindent \textit{\textbf{Classifiers' correlations show bias.}}
Figure \ref{fig:classifier} shows the correlations with community models for the five communities for different taboo classifiers with
95\% confidence intervals computed using 10,000
bootstrapped samples.
Instead of strong negative correlations, which would indicate no bias, we see several instances of positive or near zero correlations across community models and classifiers. Zero correlations while better than positive are still not ideal, since they indicate that the taboo classifier is not taking community alignment into account.
%We see averages of 0.07, 0.05, and -0.01 for Perspective, MIDAS, and NULI respectively.
 %From each community's set of comments, we randomly sampled, with replacement, to generate a new set of comments and used it to calculate the correlations between the language model and the classifier. Repeating this process 10,000 times for each community, we calculated the standard deviation of the correlations. This is shown in Figure \ref{fig:classifier}.

\begin{figure}
    \centering
    \includegraphics[width=0.75\columnwidth]{images/allThreeCorrelationsCombined-stdDev.pdf}
    %\includegraphics[width=0.66\columnwidth]{images/NULICorrelation.pdf}
    %\includegraphics[width=0.66\columnwidth]{images/MIDASCorrelation.pdf}
    \caption{Correlations of taboo classifier scores with community-language classifier scores. Error bars: 95\% confidence intervals.}
    \label{fig:classifier}
\end{figure}

NULI is relatively less biased than Perspective or MIDAS.
%But yet its negative correlations are close to low than moderate.
%These positive correlations show that the offense classifiers are not in agreement with the language models,
These correlations indicate that the taboo speech classifiers largely do not consider the language norms of the community. 

\noindent \textit{\textbf{Taboo classifiers have highest bias against the African American community.}} 
All three taboo classifiers tested show higher positive correlations for AA compared with other communities. %Showing correlations of 0.15, 0.10, and 0.05, for Perspective, MIDAS, and NULI respectively.
This disagreement with the AA community model reflects bias in the classifiers, an observation that is consistent with
those made in prior  literature
%which also showed that hate speech classifiers are biased against AA English
\cite{davidson-etal-2019-racial,sap2019risk}.

\noindent \textit{\textbf{Perspective shows highest bias.}}
%The publicly available api, 
On average, Perspective, is the least in accordance - having the most positive correlations - with the CLC models. When compared with MIDAS and NULI, the only community model for which Perspective has a lower bias is HA. This is particularly concerning as Perspective is publicly available and has already been deployed to monitor comment sections \cite{HowElPa30:online,NYTimesPersp:online}.


%\subsection{Dataset Bias Assessments}
%\label{sect:datasets}
%\subsubsection{Datasets tested}




\begin{table}[]
    \centering
    \footnotesize
    \begin{tabular}{c|c|c|p{1.5cm}}
         Dataset & Labels & Sizes & Prior Work \\\hline\hline
         Davidson & Offense & 20716 & Sap \citeyearpar{sap2019risk}\\
         \citeyearpar{davidson2017automated} & Hate & 1537 & Davidson \citeyearpar{davidson-etal-2019-racial}\\\hline
         OLID \citeyearpar{zampierietal2019OLID} & Offense & 4640 & None\\\hline
         SOLID \citeyearpar{rosenthal2020largeSOLID} & Offense & 3002 & None\\\hline
         Gab \citeyearpar{kennedy2018gab} & Hate & 2337 & Jin \citeyearpar{jin2020efficiently} \\\hline
         Founta & Hate & 27150 & Sap \\
         \citeyearpar{founta2018large} & Abuse & 4965 & \citeyearpar{sap2019risk} \\\hline
         \multirow{2}{*}{Wiki Toxic}\tablefootnote{\url{kaggle.com/c/jigsaw-toxic-comment\\ -classification-challenge}} & Toxic & 15295 & Vaidya \\
         & Hate & 1405 &\citeyearpar{vaidya2020empirical} \\\hline
         Waseem \citeyearpar{waseem-hovy-2016-hateful}& Sexist & 2673 & Davidson \citeyearpar{davidson-etal-2019-racial}\\\hline
    \end{tabular}
    \caption{Details of examined datasets. Samples of prior work which also examined these sets for bias are indicated in the final column.}
    \label{tab:datasets}
\end{table}
% pertain to bias, added to table description.
%\textbf{these cites of also studied pertain to bias studies or something else?}

%\textbf{true still??} Yes -2/6/21
%
%If for a dataset its posts disproportionately align with a community's language model then it indicates dataset bias against that community.
%The seven source datasets are listed below.


%
%
%As a reminder,
%we use a threshold on membership scores \textit{k} = 0.85.
%That is if a community's language models estimates a probability $\geq$ 0.85 then the text is viewed as using language that is acceptable by that community.
%

\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{c||c|c||c|c||c||c|c||c|c||c}
            & \multicolumn{2}{|c||}{Davidson} & & & Gab & \multicolumn{2}{|c||}{Founta} & \multicolumn{2}{|c||}{Wiki Toxic} & Waseem \\\hline
         CLC & HATE & OFF & OLID & SOLID  & Hate & Hate & Abuse & Toxic & Hate & Sexism\\\hline
         NA & 14.0 & 3.9 & 3.4 & 1.4 & 7.6 & 4.4 & 3.9 & 8.0 & \textbf{13.3} & 5.1\\
         HI & 5.5 & 5.2 & 8.3 & 3.5 & 5.5 & 5.4 & 6.6 & 4.9 & 6.3 & 3.9\\  
         HA & 4.3 & 3.1 & 6.3 & 5.1 & 3.9 & 6.0 & 4.6 & \textbf{9.4} & 3.4 & 4.2\\
         SA & 4.2 & 2.2 & \textbf{16.3} & 5.8 & \textbf{25.4} & 14.5 & 5.4 & 8.5 & \textbf{13.0} & 13.9\\
         AA & \textbf{20.7} & \textbf{29.9} & 15.2 & \textbf{30.4} & 12.2 & \textbf{32.6} & \textbf{22.5} & 4.9 & 5.3 & \textbf{45.5}\\\hline
         %Popular & 92.5 & 89.8 & 97.2 & 84.6 & 95.0 & 97.9 & 97.3 & 90.7 & 85.3 & 99.4\\\hline
         %Average & 28.0 & 22.4 & 24.5 & 21.8 & 24.9 & 26.8 & 23.4 & 21.1 & 21.1 &  28.7 \\\hline
         %Average (excl. Pop.) & 9.7 & 8.9 & 9.9 & 9.2 & 13.2 & 12.6 & 8.6 & 7.1 & 8.3 & 14.5\\\hline
         %Std. Dev. (excl. Pop.) &  7.4 & 11.8 & 5.6 & 11.9 & 8.7 & 11.9 & 7.8 & 2.1 & 4.6 & 17.8\\\hline
         
         Average& 9.7 & 8.9 & 9.9 & 9.2 & 13.2 & 12.6 & 8.6 & 7.1 & 8.3 & 14.5\\\hline
         Std. Dev.&  7.4 & 11.8 & 5.6 & 11.9 & 8.7 & 11.9 & 7.8 & 2.1 & 4.6 & 17.8\\\hline
        % BlackPeopleTwitter & 47.8 & 61.6 & 26.3 & 41.6 & 49.4 & 19.6\\\hline
    \end{tabular}
    \caption{Proportion of  Taboo datasets with high alignment scores for each CLC. Note, a given text may have high alignment with 0 or more communities. Thus column proportions need not sum to 100.}
    \label{tab:datasetBias}
\end{table*}
%\vspace{-0.5em}





%\begin{itemize}
%\noindent\textbf{Davidson} \cite{davidson2017automated}: We use two datasets of 20,716 offensive tweets and 1,537 hatespeech tweets. These were also studied by \citet{sap2019risk} and \citet{davidson-etal-2019-racial}.

%\noindent\textbf{OLID} \cite{zampierietal2019OLID}: Composed of offensive and non-offensive tweets used in OffensEval 2019/2020 \cite{zampieri2019semeval, zampieri2020semeval}. We examine the 4,640 offensive tweets.
    
%\noindent\textbf{SOLID} \cite{rosenthal2020largeSOLID}: Expanded version of OLID, constructed via democratic co-training of models. Contains 3,002 offensive tweets.

%\noindent \textbf{Moderated Reddit comments} \cite{chandrasekharan2019hybrid}: A set of moderated comments from Reddit compiled and processed to identify the reasons for moderation using topic models. 
%We take the subset of comments removed for offensive, hateful, or abusive language. This set contains 35,413 comments.

%\noindent\textbf{Gab Hate} \cite{kennedy2018gab}: 27k posts from Gab\footnote{https://www.gab.ai/}. We examine 2,337 posts labeled hateful by a majority of annotators. This set was also studied by \citet{jin2020efficiently}.

%\noindent\textbf{Founta} \cite{founta2018large}: Dataset containing 27,150 hateful tweets and 4,965 abusive tweets. These were also studied by \citet{sap2019risk}.  

%\noindent\textbf{Wiki Toxic}: Comments from the Kaggle toxic challenge\footnote{\url{https://www.kaggle.com/c/jigsaw-toxic-comment\\ -classification-challenge}}. We examine 15,294 toxic and 1,405 identity\_hate texts. This set was also studied by  \citet{vaidya2020empirical}.

%since it shows higher alignment with the Native American and South Asian models. \textbf{why refer to alignment at this point. for each itemized data source specify clearly how many and what datasets you derive.  see what i wrote for founta. there should be 10 datasets in the end}.

%\noindent\textbf{Waseem} \cite{waseem-hovy-2016-hateful}: A dataset composed of sexist and racist tweets. We study the 2,673 accessible sexist tweets. This was also studied by  \citet{davidson-etal-2019-racial}.

%\end{itemize}



\subsection{Dataset Bias Assessments and Results}
%\vspace{-0.5em}
We generate ten test sets from seven text collections annotated for taboo. A test set consists of instances labeled with one taboo label (such as hateful, offensive, sexist etc.). A summary of the datasets can be found in Table \ref{tab:datasets}.

Table \ref{tab:datasetBias} presents bias assessment results.
Each row identifies the CLC used to estimate alignment of taboo instances in the column datasets.
For example, 14\% of the texts labelled as HATE in the Davidson  dataset are highly aligned with the Native American model.
We remind the reader that we use a community classifier score threshold of 0.85 (see section \ref{sect:characteristics}). Again column sums need not be 100 as an instance may be highly aligned with 0 or more models.
The table also shows average and standard deviation. %\textbf{need horixontal line above average in table}. % (excluding the Popular model).
Cells in bold are more than one standard deviation from the mean.

As a reminder, for any community we would like the proportion of taboo labeled instances that are highly aligned with that community's language to be close to 0. 
%
Additionally, if this is not possible, we check to see if these proportions are unequal across communities.
Inequality would indicate that bias is particularly targeted at some communities - those with highest proportions. 
%

\subsubsection{Taboo text and model alignments}
\noindent \textit{\textbf{Many of the proportions are large indicating bias.}}
When examining Table \ref{tab:datasetBias}, we find that 64\% of the cells have proportions $>$ 5\%. Even with a stronger threshold of $>$ 10\% on the proportions, close to a third of the cells still exhibit bias.
%
The least biased -- closest proportion to 0, is 1.4 for SOLID gauged against the NA model. The highest is 45.5 for Waseem gauged against the AA model.
%
Examining each dataset, we see that all have large proportions of taboo text that are highly aligned with at least one community; some datasets are biased against two communities.
%
For example, Wiki Toxic - Hate has high proportions when gauged against both NA and SA.
%
When examining averages across datasets Waseem is the most biased (average of 14.5), followed next by Gab.
Wiki Toxic - Toxic is the least biased --- with the lowest average.
%HI is the least biased against community with all datasets having $\leq 8.3$ proportions.
%
Overall, all datasets  exhibit biases with proportions that are far from 0.




\subsubsection{Uneveness of alignment proportions}
%\vspace{-0.5em}

\noindent\textit{\textbf{Datasets are heavily biased against African Americans.}}
%
As seen in table \ref{tab:datasetBias}, six out of the ten datasets have disproportionate high-alignment with the AA CLC model with a seventh (OLID) coming close to crossing the 1 SD mark.
%
The two datasets with lower than average proportions are from the Wiki Toxic collection.
%
The highest proportions are with the Waseem dataset 
followed by the Founta Hate dataset.
%
Telling too is that the top six in bias have more than 20\% of their instances highly aligned with the AA model.
%
This level and consistency of bias against the AA model is remarkable. 
%It is noteworthy that the datasets which show the greatest bias against AAs are composed of tweets. 
%\textbf{this is only for the first four.  are they all tweets?}
%
%%%
%
% THIS IS WRONG! In their work, Sap et al. \cite{sap2019risk} used the false positive rate of classifiers to analyze bias in the the Davidson dataset. They found that the classifiers trained on the dataset falsely associated an offensive label with 46.3\% of the non-offensive language that was associated with the AA Language. However in only 0.8\% of the cases did it wrongly associate a hate label with the AA Langauge. 
%One explanation in the discrepancy between our result and theirs, with regards to the hate data, can be attributed to the fact that our method is focused on learning the norms of the community and not hate specifically.  
%\textbf{Osama: need some comparison with other results here - in particular Davidson, table2? and Sap figure 2 left, \\ OSAMA: We can't make this comparison, Our results are focused on how much of the total hate dataset was associated with the AA community, while theres is focused on how much of the non-hate AAE data was misclassified}
%
%This trend continues to be observed for the other datasets as well.
%
%SOLID is also heavily skewed against the AA language, with 30.4\% membership, higher than any other community. For OLID, AAs label the second highest membership with 15.2\%.
%
%For the Gab hate %dataset, AAs claim the second highest membership at 12.2 \%. 
%
%The Reddit Moderated dataset can be considered the least biased since on average $<$8.0\% of the norm violating language is associated with any particular community's core language.
%


\noindent\textit{\textbf{Datasets also biased against South Asians.}} Next to the AA community, the largest bias is against the SA community.
%
This community takes the top position with Gab Hate;  over a fourth of the data is highly aligned with the  community (25.4\%). 
%
Looking down the column this proportion for SA stands out, with the next highest --- AA, at 12.2\%.
%
In OLID and Wiki Toxic Hate, SA proportions are more than 1 SD from average.
%
SA alignments are lower than average for 5 datasets such as Davidson and 
Founta Abuse.
%
This analysis brings to light that bias is not limited to the AA community, but extends to other communities as well.
This is noteworthy as previous works such as \cite{davidson2017automated,sap2019risk} have solely focused on the bias against AA while ignoring others like SA.
%The classifiers are not biased against the communities but against the languages of the communities. 
%As discussed in section \ref{modelValidation}, the SA community's language has a significant overlap with the AA community's language. %This could also be a reason for observing these trends with SA.
%The classifiers seem to be biased against the communities that share an AA mode of communication.

\noindent\textit{\textbf{Low bias communities exist.}}
The HI and HA communities face less bias in comparison with AA and SA.
%
%In terms of alignment, both HI and HA find less than 10\% of data highly aligns with their language across all datasets.
%
In fact, for HI the proportions are lower than average across all datasets.
%
%\textcolor{red}{
%NA has 2 datasets (Davidson - %Hate, Wiki Toxic - Hate) greater than 13\% alignment, with 1 of those having
NA has proportions 1 SD higher than average for one dataset: Wiki Toxic - Hate. 
%
Otherwise, the alignment proportions are almost always lower than average.

%\vspace{0.05in}
\noindent\textit{\textbf{Results are largely comparable with previous bias results.}}
Comparisons are limited as prior work largely focuses on bias towards AA.
We make the following general observations.

%\citet{davidson-etal-2019-racial} and \citet{sap2019risk} both examine classifiers trained on the Davidson, Founta, and Waseem sets.
%We obtain mostly similar results. 
Our results are generally consistent with those of \citet{davidson-etal-2019-racial} 
and \citet{sap2019risk} on the Davidson dataset. 
E.g., all three find high rates of AA tweets as labelled offensive (between 17\% and 46\%).
We observe similar agreements for the Founta and Waseem sets.
There exists some disagreement, however, where we find the ``hate'' labeled portion of Davidson and Founta datasets to show bias against AA, while \citet{sap2019risk} did not. 
The reasons for this difference are unclear.
However, it is puzzling to note that \citet{sap2019risk} found bias against a community for one taboo class (offense) but not another (hate). The authors do not provide an explanation for this.


%For classifiers trained on the Davidson dataset, \citet{davidson-etal-2019-racial} find \textcolor{red}{17.3\% and 4.9\% of tweets to labeled as offensive/hateful respectively, 
%higher percentage of AA aligned tweets likely to be labeled as ``hate'' compared to White aligned tweets, 
%while \citet{sap2019risk} find 46.3\% of AA tweets to labeled as offensive.}
%are more than twice as likely to be labeled as ``offensive'' compared to White aligned tweets.
%We also find high percentages aligned with AA: 29.9\% and 20.7\% of Davidson offense and hate labeled sets.


%For classifiers trained on the Founta set, 
%\citet{davidson-etal-2019-racial} find a higher classification rate of AA tweets as hate and abusive when trained on the Founta set. compared to White tweets, while \citet{sap2019risk} find that the classifier labels nearly 50\% of non-offensive AA tweets as being offensive. 
%For classifiers trained on the Waseem set, \citet{davidson-etal-2019-racial} find the classifier is 1.7 times more likely to label AA aligned texts as sexist compared to White aligned texts.
%We see many similar observations in our own experiments: We find that our AA language model labels 45.5\% of the Waseem sexist labeled data, 29.9\% and 20.7\% of the Davidson offense and hate labeled sets respectively, and 32.6\% and 22.5\% of the Founta hate and abuse labeled sets as aligning with its language. 
%We do find some disagreement however, where we find the ``Hate'' labeled portion of Davidson to show bias against AA, \citet{sap2019risk} did not.

\citet{huang-etal-2020-multilingual} 
%measure bias using a fairness evaluation which involves measuring the equality differences of true positive/negative and false positive/negative rates for each demographic characteristic (e.g. race). 
examining the Waseem and Founta datasets for bias against race find BERT to show the least bias compared to CNN and RNN based classifiers. Our results are consistent as the BERT based classifier, NULI, shows lower bias than MIDAS, which is an ensemble of a CNN, and BLSTM/BGRUs. %\textcolor{blue}{good find}



Overall, our results indicate that the datasets are largely insensitive to the norms of African Americans (overwhelmingly so) and then to the South Asian communities.
Subsequently, taboo classifiers built on these datasets are more likely to be biased against these two communities.
%\vspace{-.5em}

%\vspace{-0.5em}
\subsection{Small scale user study}
%\vspace{-0.5em}
We present a small scale user study intended only to illustrate our main hypothesis, that 
texts highly aligned with a CLC should be less likely to be considered taboo from the perspective of members of that community. %We explore this with a small scale user study divided into two parts exploring classifier and dataset bias.
A rigorous user study with intra and inter community judgements and many judges is left for future work.
%

\noindent
\textbf{{Classifier bias.}} Focusing on Figure \ref{fig:classifier}, we selected a mixture of comments from OLID/SOLID and from reddit that had the highest model alignment scores ($>0.85$) with their respective CLCs. We selected 80 comments for AA and 78 for SA, all of which had high taboo classifier confidence scores ($> 0.76$) with MIDAS and Perspective, i.e., they contributed the most to the positive correlation bars in the graphs. %see that both Perspective and MIDAS are biased against AA and SA communities. To understand this bias further, 
We asked two African Americans and two South Asians, who were active Reddit users, to judge their respective sets as offense/hate or not. The annotators were selected by word of mouth. 
Given high alignment we expect annotators to contradict the classifier and judge these as not taboo.
%The extent to which this occurs is the extent of support for our language model based approach for bias detection. 

As expected, both SA annotators disagreed with the classifier assigned taboo labels in 60/78 cases (76.9\%) agreeing only in 3/78 comments (3.8\%) and giving mixed judgements in the remaining 19\% of comments.
AA  annotators
disagreed with the classifiers for 27/80 (33.8\%) comments. While non trivial, this percentage is noticeably less than 76.9\% for SA. They agreed with the classifier's taboo decision 31/80 times (38.8\%) and gave mixed judgements in 25\% of cases (more than for AA).  
Overall, judges contradicted the classifiers 55\% of the time.

\noindent\textbf{Analysis of classifier contradictions.}
In a majority of the contradictions the  classifier did not recognize benign contexts of words such as `fuck' and `shit'. E.g., in SA are: \textit{``how the fuck are Indians minorities'} and \textit{`how is an accent shitty''}. From AA: 
%\textit{``thank you I should not have said all men just the assholes at work''} and
\textit{``... drop this fake ass bitch and move on''}.
Annotators did not label these as offensive.

A second reason for contradictions appears to be because culturally subtle contexts are challenging for classifiers. 
Both SA annotators marked the comment \textit{``this is exactly the reason i don't fuck with Biryani"} as non-taboo. The classifier does not recognize this as a statement on the authenticity of a food item -   `Biryani', a rice-based South Asian dish.  
Similarly the AA annotators marked:  \textit{``I'm so fucking tired of side chick culture''} as not taboo.  The classifier does not recognize this as a critique of  extra-marital intimacy and not an attack on a `culture'. Note that all these statements have model alignment scores that are very high ($> 0.94$).

\noindent\textbf{Dataset Bias.}
Focusing on 
OLID (biased against South Asians) and SOLID (biased against African Americans), see table \ref{tab:communities}, we explore if community consistent judges will contradict dataset annotations.
We selected 
50 SOLID and 23 OLID tweets annotated in the datasets as taboo and with CLC model alignment score $\geq 0.85$. 


%We performed a similar small scale user study using the same annotators to explore dataset annotation bias. We limited this to the datasets OLID (biased against South Asians) and SOLID (biased against African Americans), see table \ref{tab:communities}. Both datsets are used as gold standard in the popular OffensEval initiative \cite{zampieri2019semeval, zampieri2020semeval}. Our goal was to see if tweets with negative class labels but with high alignment scores in the respective language model were or were not judged as taboo by members of the same community. 
%Given the premise behind our approach, we expect these to be judged as not taboo.
%datasets that were highly 
%We do not consider the Waseem dataset (with much higher bias for AA) as it is known to have author bias; more than 70\% of its sexist tweets are from 2 authors \cite{wiegand2019detection}.
%We also do not consider Gap Hate because \textcolor{blue}{Osama add}.

%There were 50 SOLID and 23 OLID tweets that were annotated to the negative class and with alignment score to the corresponding language model $\geq 0.85$. 
%As before they were asked to label the tweet as offensive or not based on the language norms of their self-identified cultural/ethnic/racial background. %The annotators were given the option to opt-out if they found the content to be too coarse or disturbing.
Both AA annotators contradicted taboo annotations for 66\% (30/50) SOLID tweets and  agreed with only 9/50 (18\%).  They mutually disagreed on the remaining 11 tweets.
Both SA annotators contradicted  83\% (19 of 23) of OLID taboo annotations. They mutually disagreed on the remaining 4.
Overall 67\% of community-specific annotator decisions contradicted taboo annotations. These contradictions are also illustrative of  our expectations of `not taboo' decisions for high alignment posts.

%\newpage
\noindent\textbf{Analysis of annotation contradictions.}
%A table of examples is included in the \textcolor{red}{appendix Should we add mention of github?}.
AA annotators chose `not taboo' in several SOLID cases based on context and their norms.  E.g., \textit{``this bitch just cut her hair short by herself''}. Perhaps the presence of language likely considered offensive in a more general setting  resulted in the taboo label.
In another example, the AA annotators contradicted the SOLID taboo label for the tweet \textit{``Niggas be so depressed on this lil app ...''}. %If this tweet was uttered by a non-AA individual, it might indeed be considered derogatory and taboo. 
We see a similar phenomenon with the SA annotators. For example, they contradicted the taboo label for the tweet \textit{``All these sick ass ppl from school gave me something and now I have to chug down this nasty drink so it can go away''}. 

Additional examples of contradictions by AA and SA annotators are in the appendix (B and C).
While a larger user-level study with suitable controls is planned for the future, these preliminary results illustrate our hypothesis that using a community perspective on taboo decisions is important and that this can be achieved using CLC model alignment scores.

%\vspace{-0.5em}
\subsection{Bias mitigation - initial thoughts}

Our empirical results and case study illustrate a potential approach for bias mitigation.
The idea is to include `reset' strategies for taboo classifiers and for annotations.
If an instance that is classified or annotated as taboo has high alignment score with a CLC then a reset strategy is invoked to examine the  decision further.
%
This can be manual analysis by a community member knowledgeable of its norms and contexts - a step that can be labour expensive.
%
Alternatively, a downstream algorithm that is more community centric may be invoked - a step that may computationally more expensive. 
%
We plan to explore these in future.

%\vspace{-0.5em}
%we can observe that the classifiers are insensitive to the context of the comments. They seem to be labeling comments that contain words with stereotypically negative connotations like 'shit','ass',bitch','fuck' etc as being offensive, even when the words are being used in a positive context.

%We note a similar trend in the datasets used for offense evaluation, especially SOLID. Most of the comments that the African American annotators found to be benign contained words that had stereotypically negative connotations. We also observe that the South Asian aligned comments labeled by OLID as offensive were political in nature. Unlike OLID, the South Asian annotators did not find offense in the political comments. 





==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/casestudy.tex <==
\section{Case Study}
As a case study, we gather a portion of moderated comments from subreddits which are part of one of the communities we tested. 
% 
Since these comments are moderated, we should expect the community language models to give lower scores to these comments, as moderators should be acting as \textit{taboo} language removers\footnote{Note: \textit{taboo} language is not the only reason comments may be moderated on a subreddit.}. 
%
For each subreddit, we check the membership scores for the community of which it belongs. That is, the data of r/LatinoPeopleTwitter is checked against the Hispanic community language model. 
%
We compare the average language model score on the test set used for verifying (section \ref{sect:verification}), against the average of the moderated comments of a subreddit. These results can be found in table \ref{tab:casestudy}.


\begin{table*}[]
    \centering
    \begin{tabular}{c|c|c|c}
         Subreddit & Community & Moderated Text Average & Community Text Average  \\\hline
         LatinoPeopleTwitter & \multirow{2}{*}{Hispanic} & 66.9 & \multirow{2}{*}{78.9} \\
         asklatinamerica &  & 77.0 &\\\hline
         ABCDesis & South Asian & 82.4 & 78.4 \\\hline
         Hawaii & Hawaii & 58.7 & 77.8 \\\hline
         NativeAmerican & \multirow{2}{*}{Native American} & 85.1 & \multirow{2}{*}{71.8} \\
         IndianCountry && 66.8 & \\\hline
         blacklivesmatter & African American & 42.0 & 80.7 \\\hline
    \end{tabular}
    \caption{Comparison of average language models scores of comments composed of moderated comments from a subreddit with the community test sets in section \ref{sect:verification}. Each subreddit's moderated comments are scored with the community language model to which it belongs. }
    \label{tab:casestudy}
\end{table*}


\noindent \textbf{Community Language Models give Lower Scores to Moderated Comments.} We observe that across communities, the community language models score the moderated text lower than the community's test set. 
%
For example, for African American, the average community test score is 80.7 compared to a score of 42.7 for the moderated comments from the subreddit r/blacklivesmatter. 
%
One exception is South Asian, which could indicate that their moderation standards are not easily agreed upon by that community. 


==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/conclusion.tex <==
\section{Limitations and Conclusions}
%\vspace{-0.7em}

%\vspace{-1em}
%
%Without the community perspective, biases in taboo classification and annotation are bound to arise.
%
%should be in accordance with the norms of the community to which the author of the text belongs.
%A community is the best judge of its norms and mores. 
We presented a new methodology for studying bias in taboo text  identification.
%
Its strength is that it is centred on community language norms - a strategy consistent with \cite{blodgett-etal-2020-language} to consider social hierarchy when studying bias and natural languages.
%
Using it we assessed the extent to which biases against
five minority communities are present - both in classifier taboo decisions and in dataset taboo annotations.
%
We found many instances of  bias with
the community most targeted being African Americans.  
%
But we also found significant biases against others such as South Asians.
%
Notably, Hispanics seems least affected though there was to some degree classifier bias.
%
%Using these language models we introduce a novel method to assess the prevalence of bias in taboo classifiers and taboo labelled datasets.
%The prevalence of bias in these other communities was less than for African Americans.
% 
%One strength of our approach is that it can be extended to any community whose members have a shared language. 
%\textcolor{red}{THIS IS IFFY}We validated our models by comparing them to already existing datasets.

%We found strong biases against African Amerians both in classifiers and in datasets.  
%We also found strong bias, but in fewer instances against South Asians.  
%that 9 out of the 10 datasets used in the previous literature to build taboo language classifiers had disproportionately high alignment scores with the African American language and South Asian language norms.
 
%
%Similarly, we used our language models to show that SOTA toxicity and hate speech classifiers were more prone to be biased against the African American community. Additionally, 2 of the 3 classifiers were also biased against the South Asian community. 
%This is a significant insight because prior work has only focused on bias against the African American language.
%
A small scale `illustrative' user study provides initial support for our key idea which is that common utterances, i.e., those with high alignment with the community's language classifier, are unlikely to be viewed as taboo from that community's perspective.
%
Annotators who are community members contradicted classifier and annotator decisions in a majority of instances.
%
%we found large disagreements between the judges' decisions (who were from the same community as the text author) and the negative classifier decisions (61\%) and the negative annotations in the datasets (67\%).
%Error analysis revealed a few prominent reasons for these contradictions which could offer a way forward for mitigating bias - \textcolor{red}{for example, ensuring that the annotators are not all members of the same community and instead representative of diverse language norms.}% for example, ensuring that political alignment is not influential during annotation.
%\textcolor{red}{Other possibilities to explore in the future include strategies to reset dataset annotations and classifier decisions by considering alignment scores or by having community members judge at least those negatively labeled or classified instances that have high alignment scores with \textit{any} minority group's language model.
%}






%
%The results we find for the African American community are in accordance with those of previous works \cite{sap2019risk, davidson-etal-2019-racial}, in that hate/offense datasets were shown to contain bias against African American communities.
%

%\noindent \textbf{Limitations} 
Our work is limited to analyzing communities defined by race and ethnicity, but is generalizable; we will explore bias against other  communities in future research.
%
We also plan to conduct a large-scale user study to better understand community perspective for taboo texts.
%
We plan to 
investigate the bias mitigation strategies shown in section 4.5.
%vary. There is an especially high difference between the Native American training set (14k comments) and the other communities' training sets (35k - 51k). This difference could lead to an inadequate representation of Native American norms by the model.
%cause the Native American language model to be inadequate in representing  
%its community, and therefore be less likely to identify bias. 
%
%A deeper examination of how the different types of taboo language relate to communities could help further the understanding of bias.

%,  second limitation is how we view taboo language. Currently, we combine all taboo language into one category. However, differences exist between them (e.g. offensive language is not always hate speech). A deeper examination of how the different types of taboo language relate to communities could help further the understanding of bias.

%\noindent \textbf{Future work}
%Future work should address the aforementioned limitations. Future work should also incorporate the ideas shown here into mitigating bias. One way could be to include community language models in taboo detection systems, to help better guide them. 

==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/graveyard.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{images/LM Distribution Vs NativeAmerican.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distribution Vs. Hispanic.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distributions Vs. Hawaii.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distributions Vs. SouthAsian.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distributions Vs. AfricanAmerican.pdf}
    \caption{Distribution of probabilities from language models against their corresponding test set.}
    \label{fig:NALM}
\end{figure}


\section{Outline}
\begin{enumerate}
\item Model construction

Methods: Two methods: BERT and XLNet.
justify these.

Datasets: reddit collections - justify.



\item Model verification

expect to see probability for native group to be high than for other groups.

\begin{enumerate}
    \item 
    native test set
    
    \item
    Blodgett demographic dataset
    
    \item
    userlevelrace dataset
    
    
\end{enumerate}

\item
exploring bias 

\begin{enumerate}
    \item 
    in classifiers
    
    \item
    in datasets
    \begin{itemize}
        \item Reddit moderated data
        \item Offenseval
        \item other1
        \item other2
    \end{itemize}
    
\end{enumerate}



(must check for consistency with what others find



\end{enumerate}

%
%\subsubsection{Datasets} \label{sect:validDatasets}
%In addition to running validation tests with the held out Reddit data (see Table\ref{tab:LMTestSet}) we use two more datasets for validation.
%These are both Twitter subsets as opposed to Reddit.
%validate our language models by using three datasets.

%We verify our models on three datasets:
%\begin{itemize}
%    \item Demographic16-AA: A dataset by Blodgett et al., which contains demographic-aware topic models for AAE (African American English), White, and Other.
%    The dataset includes a HI set, however, the paper itself does not use this data due to ``uncertainty'' of what the HI model learned. Therefore, we exclude this from our validation process as well. dialects.
%This race-annotated dataset of over 56M tweets has been regarded as the gold standard of AAE language in several papers \cite{sap2019risk, davidson2019racial, groenwold2020investigating, xia2020demoting}.
%The AAE community is comparable to the African American community in our experiments. To make the models more comparable, we sample 50k AAE tweets. Using our language models, we assign alignment scores using each community model to these tweets. 
%\item UserLevelRace-AA: A dataset by Preotiuc-Pietro et al., that contains the self-reported race of Twitter users and their tweets \cite{preotiuc-pietro-ungar-2018-user}. Like with Demographic16, we sample 50k African American tweets to form our third validation dataset. 
%\end{itemize}
%
%The dataset was built using geo-located tweets matched with Census demographic data. They then use a topic modeling approach to estimate the likelihood of each race for a tweet.  
%Their validation test show that non-HI black language tweets show language properties consistent with prior research AAE language.
%The authors estimate the dialect of each tweet by using a demographic aware topic model which leverages race and ethnicity data from the census as well as geocoordinates from the user's twitter profile. 
%
%As we are relying on models trained on Reddit data to predict language belonging to communities formed on Twitter, we expect that our models would experience a degradation in their predictive powers.
%This is because norms vary across social media, even for culturally similar communities. We still expect the norms of the language to dominate over the differences in styles across social media, resulting in our African American model outperforming the other community language models.
%Note that since our models are trained on Reddit data it is possible that estimates are lower for the same community when we use the two Twitter subsets.
%This is because the language model is likely to be shaped by the nuances of that social media platform. However, we expect community norms of language to dominate over differences in styles across social media.
%\vspace{-0.5em}
%\textcolor{red}{Note: The following idea is weak!}
%Even though these datasets are extracted from different social media platforms, our notion of community platform independent. Instead we are grouping subcultures/subreddits\textcolor{red}{NOTE: Not sure which one to go with} into communities based on their shared cultural heritage and norms. 
%A language model trained on a particular platform will learn the nuances of that medium, and is expected to suffer a degradation when tested on the language of another medium. However overall, it would still be able to use the community specific signals to detect the relevant community. And on average, it will outperform the models trained on the other communities.
%\subsection{Validation results}
%We observe the membership score distribution for each community language model on its respective held out Reddit set in 


%\textcolor{green}{The reason for this cutoff is two-fold. First, a cutoff of 0.85 ensures each community language model assigns membership to > 50\% of the language in their respective test sets. Second, this is a stronger number than \cite{blodgett-etal-2016-demographic}, which set a cutoff of 0.8. }


%
%From our observations, we choose a confidence cutoff of 0.85 when deciding whether language belongs to a community. 
%

%\textcolor{green}{As noted in model construction (section \ref{}), BlackPeopleTwitter is a highly popular Reddit community which encourages diversity in its members. This popularity can also cause those who interact with its post to fluctuate}[NOTE: We aren't running experiments to support any claims about the membership makeup of a community]. \textcolor{green}{ This led us to include it in its own model. }


%\textcolor{red}{As noted in model construction (section \ref{}), the popularity of BlackPeopleTwitter on reddit encourages diversity in its membership. This lack of homogeneity means that BlackPeopleTwitter is a community that is distinct from the other African American communities. }

%[NOTE: I HAVE SOME ISSUES/QUESTIONS. I Will engage with BPT after those have been resolved.]
%
%The distribution of memberships scores seems to reinforce this idea of diversity and fluctuation in the BlackPeopleTwitter community. 
%
%A highly diverse/fluctuating community, would not settle on common language, thereby making it difficult for a language model to learn language for that community.
%
%Because of these observations, we do not include BlackPeopleTwitter scores in the main analysis discussions going forward. 
%\par\textcolor{green}{We also test each community language model on the test sets for the other models to ensure that our models are not assigning high membership scores to all languages. These results can be found in table \ref{tab:LMTestSet}.}

==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/introduction.tex <==
\section{Introduction}
%\vspace{-0.5em}
%Rough

%Members of communities not only share interests, but also share a language}.
Members of a community rely on a shared language for communication, one which evolves naturally, \textit{in situ}, and is shaped by the norms and mores of the community \cite{gumperz1968speech}.
Norms promote \textit{Entitativity}, %\cite{universityprinciples}
the perception of group identity % and they protect members by preventing harmful utterances
\cite{allan2006forbidden}.
Norms may be explicit and codified into law or so subtle that while members may be unable to specify them they can still recognize violations \cite{chandrasekharan2018internet}.
%\textbf{Define Taboo}
Utterances violating a these norms may be considered \textit{taboo} from that community's perspective.\footnote{We include hate, offense, sexism, toxicity, and abusive utterances in \textit{taboo} while acknowledging their nuanced differences \cite{fortuna2020toxic}.}  
%
%Taboo utterances risk condemnation or even expulsion through moderation and self-regulation by  communities \cite{allan2006forbidden}. %Individuals generally try to avoid taboo language and behavior, unless there is malintent.\textcolor{red}{Do we have a cite for this?} 
%
 
%
Communities often self-regulate by censuring norm violating \textit{taboo} language %that it considers taboo 
\cite{allan2006forbidden}.  This censuring may be subtle such as ignoring taboo utterances leaving the individual somewhat isolated and ineffective. %This may be reflected for instance in the social network structure around such individuals.
Self-regulation could also be explicit and even severe such as expulsion from the community.

\noindent \textbf{Taboos are community-specific:}
Perceptions of taboos in language use are influenced by community 
%\footnote{Some taboos such as the taking of human life are largely accepted across communities.} %There is no such thing as an absolute taboo.
\cite{allan2006forbidden}.
%Different communities%, formed around race, ethnicity, geography or even gender can have distinctive norms and taboos regarding language use. %These inform their community specific notion of language taboos. 
Utterances that are benign in one community might be taboo in another\footnote{Even individuals within a community may differ in their norms and taboos, with some enforcing more constraints.}. E.g., `autistic' is considered derogatory on most of  %platforms like 
reddit, its use usually leads to censure. However, on the subreddit /r/wallstreetbets, it is not and is instead used as a self-descriptor by members.
%Multi-lingual posts raise additional challenges. A native English speaker might be consider /\textipa{bitS}/  \textit{taboo} because of its similarity to /\textipa{bItS}/. However, to a Hindi speaker, it benignly translates to `between'. %This Hindi expression may appear within a largely English utterance.
The importance of considering the author's community when studying taboo is emphasized in a recent critical survey of bias in NLP papers \cite{blodgett-etal-2020-language}; it urges us to understand how social hierarchy relates to language use.  Our research is a step in this direction.
%

\noindent
\textbf{Taboo utterance detection and biases:}
Several papers especially from OffensEval 
\cite{zampieri2019semeval, zampieri2020semeval} 
have led to the development of state of the art taboo classifiers for moderating online speech. %\cite{liu-etal-2019-nuli, Mahata2019MIDASAS, Perspective,senarath2020evaluating, arangosigir2019,badjatiya2017}.
%a range of classifiers including traditional SVM, Random Forest classifiers, deep learning models (CNN, LSTM, GRU), and transformer-based models (BERT, GPT2) have been explored.
%The general reason for identifying taboo utterances online is to moderate and reduce negative effects of toxic speech. 
%
%
%In order to grow, social media platforms need to be both inclusive of communities, but also create a place users are comfortable in. To address the latter, platforms have begun to add in automated detection algorithms for offensive and hateful language \cite{}.
%However, due to the aforementioned reasons, these algorithms can unintentionally target minority groups, thereby hurting the inclusivity of the platform. 
Alongside, an active research stream studies the presence of bias in taboo detection. % and in the annotated datasets used for training.
Biases, specifically having higher false positive rates for a minority community compared to the majority, have been detected particularly against African Americans and also to some extent women \cite{dixon2018measuring,zhou2021challenges,bolukbasi2016man,xia-etal-2020-demoting,chuang2021mitigating}.
Bias is clearly harmful as penalties over false positives could over time discourage/constrain minority participation on social media platforms, and in turn reinforce the majority's norms and values.
%[A key reason for bias is skewed representations in training data and sampling methods \cite{wiegand2019detection}, as
%for example, over-representation of identity terms in negative contexts \cite{bolukbasi2016man}. There has been good progress in mitigation strategies for such biases \cite{xia-etal-2020-demoting,badjatiya2019stereotypical}. SKIP]

%Most of the state of art taboo language detectors are limited, more specifically biased, in that they are more in tune with the mainstream language expressions and much less aware of the languages and dialects of minority communities.
%
%

\noindent
\textbf{Limitations in bias assessment research:}
A limitation is that community language norms are rarely considered.
While recent research on taboo detection discuss and illustrate the importance of community perspective  \cite{davidson2017automated, sap2019risk, badjatiya2019stereotypical} we do not yet have bias detection methods that are firmly founded on community language norms.
This methodological gap underlies not only the design of state-of-the-art taboo detection tools but perhaps more crucially even in the methodologies for the \emph{study} of bias in taboo detection. 
Not only are the taboo annotated datasets largely devoid of community, culture or social contexts (i.e., characterization)
\cite{zampieri2019semeval, zampieri2020semeval}, the study of bias itself needs strengthening with methods wherein a community perspective stays front and center, consistent with the urging in the survey \cite{blodgett-etal-2020-language}.

%However, most modern NLP systems that deal taboo language detection, especially in the form of offensive and hate speech classifiers, rely on datasets that are devoid of cultural and social contexts \cite{zampieri2019semeval, zampieri2020semeval}. The classifiers built using these context-independent datasets inevitably end up treating the taboo norms of the mainstream language as the default standard.

%It is therefore not surprising that researchers have shown that utterances from minority community members are labeled more frequently as offensive, hateful, toxic or undesirable\cite{sap2019risk, davidson2019racial}. 




%\noindent \textbf{Limitations of SOTA detectors}
%
%taboo language detection, especially in the form of offensive and hate speech classifiers, has recently been garnering much attention \cite{zampieri2019semeval, zampieri2020semeval, sap2019risk}. 
%
%Most of the state of art taboo language detectors are limited, more specifically biased, in that they are more in tune with the mainstream language expressions and much less aware of the languages and dialects of minority communities.
%
%It is therefore not surprising that researchers have shown that utterances from minority community members are labelled more frequently as offensive or undesirable [CITE]. 
%Such biases can limit participation by minority communities on social media platforms and result in great losses to people as a whole.
%

%There are at least three major reasons for such biases in taboo language detectors. First, these classifiers are trained on datasets which are heavily skewed towards mainstream communities. 
%This has been observed as a source of bias in several papers [CITE] and has implications in terms of how datasets are to be built. %not representative of minority languages. 
%
%Second, these algorithms rarely \textbf{ok to say rarely?} consider the context in which the utterance is made <insert example>. 
%An exception is where X considers the post thread.
%
%Finally, these algorithms \textbf{ok to say never? if not give me an example} never 
%take into account community specific language usage norms and mores.
%While some progress has been made with the first two reasons, there is no work yet on studying the nature of this bias through the lens of a community's language norms and taboos.
%


%and thus can be biased against minority languages and dialects. This bias shows up in hate, toxicity, and abusive language detection as well \cite{}.

%[\textbf{consider deleting why is bias bad section}
%\textbf{Why is Bias Bad?}
%This bias can then lead to censorship of minorities on social media platforms, by disallowing them to express themselves in their native styles. 
%
%In order to grow, social media platforms need to be both inclusive of communities, but also create a place users are comfortable in. To address the latter, platforms have begun to add in automated detection algorithms for offensive and hateful language \cite{}.
%However, due to the aforementioned reasons, these algorithms can unintentionally target minority groups, thereby hurting the inclusivity of the platform. ]
%

%By quantifying the bias in these datasets and classifiers, researchers have been highlighting the need to redefine taboo from a community specific perspective. However, this notion of community sensitive taboo has not be explored sufficiently.



\noindent \textbf{Contributions:} %Set in the above context we propose a new methodology for studying the prevalence of bias in taboo datasets and classifiers. Specifically:

%In this paper, we argue that notion of what constitutes taboo language should be evaluated based on the norms of each community separately. 
%\vspace{-0.25em}

%\begin{enumerate}
\noindent 1. We propose a new method that is firmly grounded on community-specific language norms for studying bias in taboo detection.
    %Specifically, we build and validate distinctive language models for communities of interest. We then use these models to study bias against those communities.
%\noindent 2. Our method can be used to study bias against different minority communities. 

\noindent 2. We use our method to assess bias against five minority communities in three taboo text classifiers and ten taboo annotated datasets.
In contrast, prior research has largely about bias against the African American community, possibly due to reliance on two race estimated/labelled datasets %Davidson \cite{davidson2017automated} and 
    %Blodgett
    \cite{blodgett-etal-2016-demographic, preotiuc-pietro-ungar-2018-user}. 
    

    
    
\noindent 3. We find, for example, that all three taboo classifiers are biased against the African American community. Additionally, 2 classifiers are biased against the South Asian communities and one against Hispanics. Overall, only 3 of the 15 classifier - community combinations tested were somewhat unbiased. 
    
\noindent 4. Eight out of 10 taboo annotated test sets are strongly biased against African Americans, while at least 3 are biased against South Asians. We did not find any remarkable dataset biases against Hispanics but we found single instances of bias against Native American and Hawaiian  communities.
%    It would follow that the norms of one community can not be used to inform the language \textit{taboos} of another. 
%\end{enumerate}


%\noindent \textbf{Paper Organization:}
%The rest of the paper is organized as follows. Section 2 describes our approach for identifying bias using community focused models. We present the construction and validation of these models in Section 3. We show bias against various communities in both classifiers and datasets in Section 4, illustrated further by a small scale user study. Section 5 discusses related work before concluding.







%In this paper, we argue that only a community is qualified to identify what it considers as taboo language. We propose a notion of community sensitive language models that are representative of the norms of the community. 

%Using these community language models we introduce a novel method, that relies of the `belongedness' of language, to quantify bias in existing datasets and taboo detection classifiers. Since the notion of `belongedness' is community-sensitive, our proposed method of bias detection is not limited to any particular community. Instead it can be used to quantify bias against any subgroup that has a shared set of norms, reflected in its language use.
%then show that As such   As such 
%
%Our work is focused on understanding community-level bias, and does not deal with bias mitigation.
%
%We take a community perspective approach to taboo detection. 
%We analyze communities formed on online social media platforms, around common cultural heritage\footnote{Subreddits from the popular social media website \url{www.reddit.com}}. 
%
%\textcolor{red}{In her work, Anna Wierzbicka discussed how language use in the form of speech acts can encode the differences in cultural norms\cite{wierzbicka1985different}. Building up on this notion, we use State-of-the-Art (SOTA) language models to represent the norms of the communities.}
%
%The probabilistic nature of these models lends itself to quantifying the representations of the norms of a community. Language that is closely associated to the community's norms is more likely to be associated with its respective language model, while the language that goes against the norms, and is thus infrequent, is less likely to be associated with the community's language model.
%
%Our goal is to use these community language models to look for bias in the datasets used to train the taboo language classifiers, but also the classifiers themselves. 

%We specifically ask the following research questions:

%As an outocme of In doing so, we ask the following research questions:

%%%%%%%%%%%%%%
%
%We train language models on 6 communities composed of identity-based<or some other word> subreddits from reddit. We show that, of the instances that were manually annotated as hate, on average only XX.Y\% were considered to be part of the community's language. In contrast, of the instances that were labelled as being taboo by the SOTA classifiers, ZZ.B\% were considered to be part of the community's language.
%

%\textbf{Research Questions}

%\begin{itemize}
%    \item Are language norms different across communities?
    %\item Is a community's notion of taboo language in line with the mainstream notion?
        %\item Does a community's language extend beyond a particular social media? (Blodgett)[Can we make this argument in the write-up]
  
 %   \end{itemize}

==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/modelConstruction.tex <==
%\vspace{-0.5em}
\section{Community Language Classifiers}
%\vspace{-0.5em}
%We present the details of language model construction (using training data) and validation (with unseen data) for each community.


\begin{table}[]
    \centering
    \footnotesize
    \begin{tabular}{c|c|c|c}
                    &No. of&   Training & Validation \\
         Community& Subreddits & set size & set size\\\hline\hline
         NA & 2 & 44k & 1.4k\\\hline
         HI & 4 &95k & 6k\\\hline
        HA & 1 & 80k & 2k\\\hline
        SA & 1 &101k & 6k\\\hline
        AA & 11  & 70k & 5k\\\hline
        %PopularSubreddits&10& r/worldnews, r/Showerthoughts, r/videos, r/gifs, r/aww, r/todayilearned, r/gaming, r/pics, r/funny, r/AskReddit & 100k & 50k \\\hline
        %Black People Twitter & 100k & 189k \\\hline
    \end{tabular}
    \caption{Dataset details for each  community.}% and the popular community.}
    \label{tab:communities}
\end{table}

%\noindent \textbf{XLNET} XLNet is an auto-regressive language model that makes use of permutation language modeling\cite{yang2019xlnet}. Unlike BERT which predicts language tokens sequentially, XLNet predicts them in a random order.
%Like with BERT, we train XLNet on each community's language. The XLNet-LM of each community is used to indicate the likelihood of a text belonging to that community. 
%In our experiments both XLNet and BERT had comparable performances. However, in our final implementation we choose BERT over XLNet since it had a higher F-Score for our task.



\subsection{Model Construction}
%\vspace{-0.5em}
We build our community classification models using BERT %-\textcolor{red}{NSP}
\cite{devlin-etal-2019-bert}\footnote{Our code and data are available at: https://github.com/JonRusert/SuumCuique}. Experiments using XLNet \cite{yang2019xlnet} gave comparable results. Thus, we only report BERT results. BERT is a transformer-based model which has shown to perform well in NLP based tasks \cite{devlin-etal-2019-bert, 9058044}. BERT leverages context (on top of words)\footnote{For example, while ``is that all you have to contribute'' and ``contribute this have that is to you all'' have the same set of words, BERT will find the former more likely.}. We fine-tune BERT-base-uncased
\footnote{Models were trained on GeForce GTX 1080 Ti's, and took at most 3 hours to train. Parameter configuration is that of base-BERT, we use a dropout of 0.3 before the linear layer.}  with a linear layer on top. A softmax function is used to make a binary classification as to whether or not the input text belongs to the community. Each community has its own classifier representing its language norms. 
%When given a new text the model returns the probability of its membership in that community. We refer to these probabilities as alignment scores. Higher probabilities correspond to greater alignment with the language norms of the community.


We build our models with publicly available data from select subreddit comments obtained using Pushshift \cite{baumgartner2020pushshift}\footnote{In our experiments, we do not use any data beyond that which is available on Pushshift. Pushshift is a public Reddit data repository.}.
%
We group subreddits into communities based on shared cultural/ethnic heritage
determined using subreddit descriptions (subreddits are listed in appendix A). While we acknowledge that subreddits are not inclusive of all members of communities of interest, they can still be considered as fairly representative in terms of language use.
We do not have to be exact about the data used to represent a community
as long as we are confident that the collection is mostly produced by its members\footnote{We also acknowledge that Reddit itself has some language norms. However, these norms should apply across all of our community subreddit datasets and so should not influence our results in significantly.}.
%We run validation tests.

%
We build models for: Native American (NA), Hispanic (HI), Hawaii (HA), South Asian\footnote{South Asian English is considered non-standard compared to mainstream English.}%, thus we include this as a  ``minority' group.} 
(SA), and African American (AA) communities.
%
We obtained comments from 2018 using the first 11 months as training data for the models and the last as validation. 
%
As the data for NA was smaller than the rest, we added 2015, 2016, and 2017 data again with the first 11 months for each year as training and last 1 month for validation. 
%
%Additionally, we build a language model based on the ``Popular'' subreddits. That is, we obtain comments from the top 10 subreddits, where top is defined by the number of subscribers. Since the amount of comments is much higher for the popular subreddits, we took a sample of 50k comments for the training set and 50k comments (from the 12th month) for the validation set. 
%Note that the popular set is likely to contain posts from minority members as well.
Comments were lowercased and stripped of punctuations. 
%Each community is composed of subreddits centered around the culture of that community.
%which allude to being comprised of members mainly from that community. 
%For example, r/Hawaii is a subreddit for discussing local Hawaiian culture. 
%\textcolor{green}{r/BlackPeopleTwitter is included as its own standalone community. This is because r/BlackPeopleTwitter is a highly popular subreddit and also encourages users from all backgrounds to interact with it. The high popularity of the subreddit, means that the community will fluctuate and be diverse. This means that the community is unlikely to establish common language norms and therefore the corresponding language model will be less sure when it comes to membership of language. https://www.reddit.com/r/BlackPeopleTwitter/ NOTE: Comment on Norms encourage posts about black culture but not any restriction on who can comment}

%For African Americans, r/BlackPeopleTwitter was originally included, however, the decision was made to split this into its own community as the popularity of the subreddit seemed to indicate that the members were largely mixed. We treat r/BlackPeopleTwitter as its own community for this reason. 
Since subreddit sizes vary, the amount of data collected for each community varies as well. HI, HA, SA, and AA are the closest in size and NA the smallest. %The popular subreddits %, while r/BlackPeopleTwitter had 1.5M, which we down-sampled to 50k. 
%
%To add negative training examples, we conduct sampling from all the other communities at a 1:1 ratio of positive to negative. 
%
When training a community model we generate negative samples (texts not from the community)
by sampling  equally from the other communities till we reach a 1:1 ratio of positive to negative text samples.
%
%
%For example, while building the model for the HI community we sampled one comment from each of the other communities at a time until 47.5k negative examples were obtained.
%
%The negative are then combined with the 47.5k positive examples to produce the training set, at a size of 95k. 
%
A summary of the datasets is in Table
\ref{tab:communities}.
% 
Note that the training set size indicated includes both positive and negatives examples (at a 1:1 ratio) while the validation sets only contain positive (aligned) examples. 

\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
                    &No. of&  Training & Validation \\
         Community&Subreddits & set size & set size\\\hline\hline
         Native American & 2 & 44k & 1.4k\\\hline
         Hispanic & 4&95k & 6k\\\hline
        HA &1 &80k & 2k\\\hline
        South Asian &1&101k & 6k\\\hline
        African American&11 & 70k & 5k\\\hline
        %PopularSubreddits&10 & 100k & 50k \\\hline
        %Black People Twitter & 100k & 189k \\\hline
    \end{tabular}
    \caption{Dataset details for each minority community and the popular community.}
    \label{tab:communities}
\end{table}
\fi








    
 
  
    

==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/modelVerification.tex <==
\vspace{-0.5em}
\subsection{Model Characteristics} \label{sect:characteristics}
\vspace{-0.5em}
\begin{figure}
    \centering
    %\includegraphics[width=1.3\columnwidth]{images/AlignmentAll.eps}
    \includegraphics[width=1\columnwidth]{images/fig1_B.pdf}
    %\includegraphics[width=2\columnwidth]{images/nativeDistsZoomed.pdf}
    \caption{Complementary cumulative distribution function of community-language alignment scores for the five community models using the community specific validation datasets. An alignment score indicates the proportion of the community's comments that the model classifies as belonging to that community within a given threshold. The dotted/dotted-dashed lines (0.7, 0.9) show the proportion of comments at those thresholds. 
    The dashed line (0.85) indicates the chosen threshold for our experiments.}
    \label{fig:correspondingLM}
\end{figure}




%\textbf{use different line types in graph.  3 reds look the same to me.}
Figure \ref{fig:correspondingLM} presents the complementary cumulative distribution function (CCDF) of alignment scores (classifier confidence scores) for the CLCs using validation data. 
%The popular dataset stands out in that the popular model aligns close to 90\% of its texts at score above 0.90. %\textcolor{blue}{correct?} - yes
For example, 62.9\% and 66.2\% of the HA and the HI texts have scores $\geq$ 0.7.
%as belonging to their communities.
All CCDFs follow a similar distributional pattern.
%Similarly, at the 0.90 cutoff, the models manage an alignment score of 51.2\% and 55.4\% respectively.
We introduce a threshold on alignment scores to decide which texts are `highly aligned' with a model.
Higher thresholds imply fewer comments will be regarded as following the community's norms.
We choose 0.85 as threshold since at least 52\% of the comments for each community are then regarded as highly aligned (range: 52\% - 64\%). 
When we reduce the threshold to 0.65,  two-thirds of the comments are highly aligned. But this increases the risk of overlap across communities in their highly aligned comments. 
%For example, for a cutoff of 0.70, the percentages for the different communities range from 61.2\% to 74.0\%. %\textbf{add one other than 0.85}.
%give high membership scores for their respective test sets. 
%
%We observe that 40\% of data is greater than 0.95 confidence for the models.
%Crucially, we observe that more than half of the utterances from all communities have alignment scores of 0.85 or higher with the corresponding model.
%With an even higher cutoff of 0.95, most communities have half or more of their utterances highly aligned.
%We select $\geq 0.85$ as the threshold to decide if a comment is `highly aligned' with a model or not.
Taking the SA CLC model as an example in Figure \ref{fig:correspondingSA}, we can see that with 0.85 cutoff, $60.7\%$ of comments from the South Asian community are highly aligned, while including no more than $14\%$ (range: 2\% - 14\%) of comments from the other communities.
While not strictly comparable, our 0.85 threshold is more conservative than the 0.80  used in \citet{blodgett-etal-2016-demographic}. 

%As a contrast we also show \textcolor{blue}{add also are the other graphs in teh appendix or not? and see if argument in above para is ok. }.
% - we aren't allowed an appendix, can add to github link if choose so.

\subsection{Model Validation} \label{sect:verification}
\vspace{-0.5em}
Results with our validation datasets (shown in Table \ref{tab:communities}) are in Table \ref{tab:LMTestSet} with cell values representing proportions.
For example, 51.8\% of the NA validation set is highly aligned (alignment score $\geq0.85$) with its own community model.
Column values do not necessarily add up to 100\% as a text may be highly aligned to more than one community model or even to none.
%
%Diagonal entries represent the proportion of alignments of a dataset with its own community model -
%ideally these are high.
%Off-diagonal cells show validation data gauged against other community models - ideally these are low.

%
%The first observation to make is that all validation sets have low alignment scores with the `popular' language model; proportions are less than 1\%.  This emphasizes that the language used in the minority communities are distinct from the one-size-fits-all general model. 
%This reinforces our motivation which is to adopt community sensitive methods for detecting bias.

As expected, proportions at the diagonal representing homogenous model - dataset combinations  are high, ranging from 52 to 64\%. 
%
%E.g., the HI model assigns high alignment scores to 58.2\% of its own validation set and to less than 5\% of the validation data from other communities. 
%
%
Also as expected, the off-diagonal entries representing heterogeneous combinations,   are low. Most are less than 10\% and more than half less than 6\%. The three noticeable exceptions are between AA and SA and also between NA texts and the HA model. 
%20.7\% of the AA text are aligned with the SA model and conversely 14.4\% of the SA texts are aligned with the AA model.
%Similarly, 15.1\% of the NA texts align with the HA model.
The sociological literature
observes linguistic exchanges between minority communities  \cite{bucholtz1999borrowed,coleman1998language,igoudin2011asian,lee2011globalization}.
For example, 
\cite{shrikant2015yo}
discuss a tendency of South Asians to adopt the features of African American Vernacular English (AAVE).
This is particularly relevant to the AA and SA overlaps. Next we use these validated models to estimate bias in classifiers and in datasets.
%may explain some of the non diagonal values being above 5\% for instance.

%The overlap we observe possibly reflects this trend. 
%
%In general looking at the row for the African American model we find that the average amongst off-diagonal proportions (excluding SA) is 8.95\%.



%
%Finally, 14.8\% and 15.7\% of the Popular texts align with the HA and AA models respectively. As the Popular model encompasses users from all parts of Reddit, it makes sense that some language of the smaller communities would appear. 

%
%Results with the AA aligned tweet datasets are both similar and different. We remind the reader that we only have African American test data for these two tweet datasets. Around 30\% of the tweets are highly aligned with the source AA model.  While the proportions are low as expected  with the other minority community models, large proportions are aligned with the Popular model. A possible explanation is that the method for tagging these datasets by race is itself approximate. However, this does not hold for Race-AA dataset which is based on harvesting self-reported race.We suggest that the high proportions for Popular may be because of differences in the two media, e.g., the tweets are smaller and they are posted to a more general forum as compared to the subreddit data used to build the models. We will explore this line of analysis in future research.
%
\iffalse
\begin{table*}[h]
    \centering
    \begin{tabular}{c||cccccc}
        & \multicolumn{6}{|c}{Reddit Validation  Sets} \\\hline
         & Native &  &  & South & African & \\%&  Demo- & UserLevel\\
         \textcolor{red}{Community-}Language Model & American & Hispanic & Hawaii & Asian & American & Popular \\ \hline %&  graphic16-AA  & Race-AA   \\\hline
         NA & \textbf{51.8} & 1.8 & 4.5 & 1.8 & 2.2 & 3.4 \\%& 0.9 & 6.3 \\
         HI & 4.3 & \textbf{58.2} & 2.1 & 2.3  & 2.2 & 2.8 \\%& 4.3 & 4.8 \\
         HA & 15.1 & 6.2 & \textbf{58.1} & 5.1  & 6.9 & 14.8 \\%& 8.0 & 12.8\\
         SA & 6.1 & 5.2 & 5.8 & \textbf{60.7} & 20.7 & 7.5 \\%& 3.4 & 6.8\\
         AA & 9.8 & 7.1 & 8.1  & 14.4 & \textbf{64.0} & 15.7 \\  %& 29.8 & 31.1\\
         Popular & 0.1 & 0.4 & 0.1 & 0.2 & 0.1 & \textbf{87.6} \\%& 78.8 & 92.6\\ 
         \hline
         %BlackPeopleTwitter & 3.3 & 3.7 & 7.0 & 6.6 & 26.3\\
    \end{tabular}
    \caption{Proportion of each validation set that is highly aligned with each community\textcolor{red}{-}language model. An alignment score threshold of 0.85 is used to determine high alignment. A text may be aligned with 0 or more models, so column numbers need not sum to 100.}
    \label{tab:LMTestSet}
\end{table*}

\fi
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{c||ccccc}
        & \multicolumn{5}{|c}{Reddit Validation  Sets} \\\hline
         %Language & Native &  &  & South & African \\%&  Demo- & UserLevel\\
         %Model & American & Hispanic & Hawaii & Asian & American  \\ \hline %&  graphic16-AA  & Race-AA   \\\hline
         CLC & NA & HI & HA & SA & AA\\\hline
         NA & \textbf{51.8} & 1.8 & 4.5 & 1.8 & 2.2  \\%& 0.9 & 6.3 \\
         HI & 4.3 & \textbf{58.2} & 2.1 & 2.3  & 2.2  \\%& 4.3 & 4.8 \\
         HA & 15.1 & 6.2 & \textbf{58.1} & 5.1  & 6.9  \\%& 8.0 & 12.8\\
         SA & 6.1 & 5.2 & 5.8 & \textbf{60.7} & 20.7  \\%& 3.4 & 6.8\\
         AA & 9.8 & 7.1 & 8.1  & 14.4 & \textbf{64.0}  \\  %& 29.8 & 31.1\\
         %Popular & 0.1 & 0.4 & 0.1 & 0.2 & 0.1 & \textbf{87.6} \\%& 78.8 & 92.6\\ 
         \hline
         %BlackPeopleTwitter & 3.3 & 3.7 & 7.0 & 6.6 & 26.3\\
    \end{tabular}
    \caption{Proportion of each validation set that is highly aligned with each CLC. An alignment score threshold of 0.85 is used to determine high alignment. A text may be aligned with 0 or more models, so column numbers need not sum to 100.}
    \label{tab:LMTestSet}
\end{table}


%Overall, our validation experiments indicate that all studied minority communities have distinct norms in their language use and these are being captured by our language models.
%Also these norms are different from the norms represented by the Popular model. %The language models we developed are able to effectively distinguish between communities based on their language use.
%These observations give us confidence that the implemented community language models may be used for the next step of assessing bias. 


\begin{figure}[]
    \centering
    %\includegraphics[width=1.3\columnwidth]{images/AlignmentSA.eps}
    \includegraphics[width=1\columnwidth]{images/AlignmentSA_new.pdf}
    %\includegraphics[width=2\columnwidth]{images/nativeDistsZoomed.pdf}
    \caption{Complementary cumulative distribution function of alignment scores for all five minority community validation sets as gauged against the South Asian community's CLC. }
    \label{fig:correspondingSA}
\end{figure}


==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/relatedWork.tex <==


\section{Related Work}
%\vspace{-0.5em}

The study of bias in taboo classifiers is an active area of research \cite{wiegand2019detection, huang-etal-2020-multilingual,blodgett-etal-2020-language, park-etal-2018-reducing}.  
%
Since our focus is on bias detection we do not cover areas such as bias mitigation \cite{tsvetkov2020demoting,chuang2021mitigating} and allied problems such as bias in embedding spaces \cite{park-etal-2018-reducing,Caliskan183} and the source of bias  \cite{binns2017like,waseem2016you}.
Instead we focus on bias detection - particularly on their methodologies.
Note as most papers combine methods our binning is not intended as mutually exclusive classes.
%Since our focus is on bias detection we do not cover bias mitigation methods which is itself a vibrant subfield \cite{tsvetkov2020demoting, jurgens2017incorporating, xia-etal-2020-demoting, rios2020fuzze}.

%There are also allied research thrusts such as studying bias in embedding spaces \cite{park-etal-2018-reducing, Caliskan183} that we do not cover here.

%Also significant is research such as by Binns et al. \citeyearpar{binns2017like} and Waseem \citeyearpar{waseem2016you} who observed that the annotators' perception of taboo\footnote{offense and hate}, when building datasets, can carry biased, based on their demographics and level of expertise. 

%We do not detail this direction either. Instead


\noindent \textbf{Bias detection focused on individual words:}
%We argue that taboo should not be defined by annotators who are not part of the community, at the very least the taboos of the community should be defined in relation to its own norms.
%Works like \cite{caliskan2017semantics} and \cite{bolukbasi2016man} have shown that societal biases against particular groups are reflected in language use.
%When these tainted datasets are used to build embedding spaces, the societal biases manifest in the form of word associations. 
%\textbf{don't understand above para enough to edit}
Dixon et al. \citeyearpar{dixon2018measuring} working with Wikipedia Talk Pages show that toxicity classifiers disproportionately misclassify text with identity terms such as `gay' and `muslim' when they appear in benign contexts. % into the negative class, even when these terms are used in benign contexts.  
 A reason for this bias is because of their dominant occurrence in hateful, toxic or otherwise taboo contexts, thereby skewing training datasets. 
 %
 They show this can be countered by augmenting data with benign examples using these identity words. 
\citet{park-etal-2018-reducing}, and \citet{kennedy2018gab} also study similar biases in the data.
%Additionally, Kennedy et al. \citeyearpar{kennedy2018gab} observe that removing identity terms from testing data degrades classifier accuracy.
Badjatiya et al., \citeyearpar{badjatiya2019stereotypical} extend this analysis to words in general, finding strings like `@ABC' and `dirty' stereotypical of hate.
The general approach in these papers is to compare classifiers built from skewed and synthetically augmented/corrected non-skewed datasets.
In contrast to focusing on specific words, we analyze texts contextually with CLCs. 

\noindent \textbf{Bias detection using an external race/gender labeled dataset:}
Davidson et al. \citeyearpar{davidson-etal-2019-racial} examine five datasets including the Davidson and Founta datasets we study%\footnote{\textbf{ADD} list datasets here: (racist/sexist/ hateful/ offensive/ abusive/etc.)}  for bias against African Americans
. 
%
Their strategy is to build a classifier (regularlized logistic regressor) on each dataset and test them on the \citet{blodgett-etal-2016-demographic} black-white-race-aligned dataset.
%\citet{davidson-etal-2019-racial} used separate datasets to train th
%They trained a separate regularized logistic regressor on each dataset and used each to classify a separate dataset of black-aligned and white-aligned tweets provided by Blodgett et al., \citeyearpar{blodgett-etal-2016-demographic}.
They observed that `black-aligned' tweets were 1.8 to 2.6 times more likely to be classified as taboo.
Using similar methodology, Sap et al. \citeyearpar{sap2019risk} also found bias against AA in neural network classifiers trained on the Founta and Davidson datasets  %\citet{founta2018large} and \citet{davidson2017automated} datasets 
when tested against the same \citet{blodgett-etal-2016-demographic} dataset.
%Additionlly, they  tested their classifiers on a second race labeled 
%(here race is self declared, was this  Preotiuc-Pietro et al. dataset only labeled with AA and other?) 
% It also had Latino, Asian, and White  
%dataset by \cite{preotiuc-pietro-ungar-2018-user}.  Here too they observed biases against African American English (AAE) though not as pronounced as with the Blodgett dataset.
%In contrast to these works, our approach does not rely on race labeled datasets.


%Kim et al. \citeyearpar{kim2020intersectional} used the race alignment model from Blodgett et al., to identify AAE-leaning tweets in the Founta et al. dataset. In addition, they annotated for gender in order to study `intersectional bias'.  They found for example, that AAE tweets were 3.7 times more likely to be labeled as `abusive'.
%As in the Sap et al., paper they again did not find a difference in `hate' labeling overall.  However, when intersected with gender there was a pronounced bias against AAE male-labeled tweets; 77\% more tweets were likely to be labeled as hateful. The bias was only slight for AAE female-labeled tweets. %\texit{females}. 
%In contrast to these works, our bias detection methodology does not depend on a single race labeled dataset.

%\vspace{-0.25em}
Using a slightly different approach \citet{kim2020intersectional} trained a classifier on the \citet{blodgett-etal-2016-demographic} dataset to identify AA-leaning tweets in the Founta dataset. 
They found that AA tweets were 3.7 times more likely to be labeled as taboo.
%
Additionally, they also annotated the Founta dataset for gender. 
They found that AA male-aligned tweets were 77\% more likely to be labeled as taboo. %The bias was lesser for AA female-aligned tweets. %\texit{females}. 
In contrast to these works, our approach does not rely on access to race labeled datasets such as the \citet{blodgett-etal-2016-demographic} dataset.

%%%
%\subsection{Bias detection using synthetic datasets}

%Dixon et al., used a template approach to create a dataset of 77,000 examples with 50\% toxic instances \cite{dixon2018measuring}.
%These were used to test for model bias in datasets.
%Focusing on gender bias Park et al. \citeyearpar{park-etal-2018-reducing} use a similar approach to create a dataset of neutral and offensive instances balanced across genders. 
%They test several neural net classifiers (CNN and two versions of GRUs) trained on Waseem and Founta datasets and find that classifiers built from the Waseem dataset displayed greater bias against females than the Founta dataset. In contrast with this approach, we do not rely on synthetic datasets for assessing bias.

\noindent\textbf{Other approaches:}
As in \citet{kim2020intersectional},
\citet{sap2019risk} used classifiers trained on  \citet{blodgett-etal-2016-demographic} to identify `black-aligned' tweets in
the Founta and Davidson datasets. %\cite{founta2018large} and \cite{davidson2017automated} datasets. 
%
The difference is that they then computed correlation of probabilities of `black-aligned' tweets and the taboo language annotations and found these to be strong positive. %. They also found that the false positive rates were much higher for black-aligned tweets. %Somewhat puzzling is that the difference in FPR was unremarkable for `hate' classification in the two datasets.
We also compute Pearson correlations between classifier scores and community alignment scores. But we differ in that we are not relying on the \citet{blodgett-etal-2016-demographic} dataset.  Instead, we use alignment scores estimated using CLCs.
%It is difficult to understand why there would be bias in the other two classes and not in hate detection for the same datasets.

While the above works highlight limitations in using a single standard English model they do not propose alternative methods founded on the language norms of specific communities. We address this gap with a community-specific method using CLCs which allows us to study bias for any community. % for which we can identify, with reasonable confidence, a collection of texts. 
%
Moreover, unlike the works reviewed, and more recent papers on debiasing strategies (\citet{zhou2021challenges,xu2021detoxifying}), where the emphasis is on bias against AA, we study bias against five different minority communities.
 %This lack of examination is likely due to the lack of datasets labeled explicitly by community.
%We do not have this limitation.
%\vspace{-1em}
%Three broad approaches for assessing bias in datasets can be identified in prior work. We represent a dataset of interest by D. (1) Build a classifier on D and test it on a race labeled dataset R.  Examine the relative proportions that fall into each taboo class.
%(2) Use an approach for labeling race to label D. then use a cross validation design to build a classifier on D.  Examine the relative proportions that fall into each taboo class.
%(3) Estimate correlation between race alignment probabilities in D and gold standard annotations in D. Examine the extent to which these are positively correlated.

%Given its central role, it is important to note how this was tagged for race. Blodgett et al. matched tweet geo-location information with block level demographics obtained from the US Census. 
%They then built models  that return the probabilities of a tweet reflecting the dialects of each of four groups: non-Hispanic white, non-Hispanic blacks, Hispanics and Asians. They validated their work by showing that tweets with high probability of non-Hispanic black were linguistically consistent with prior research on AAE dialect.

%Previous works have relied on false positive rates to gauge bias, however this assumes that the training data labels themselves are not biased. However, \cite{binns2017like} in their work demonstrate that different demographics perceive offense differently. In their experiments they observed that on average female annotators find comments less toxic than their male counterparts. Similarly, \cite{waseem2016you} show that amateur and expert annotators disagree in what they consider hate speech. 

%The datasets\cite{davidson2017automated,founta2018large} use to train various taboo speech classifiers lack community based identifiers. They also lack information on the demographics of the annotators. 

%In their work, \cite{sap2019risk} show that priming the annotators about the communal provenance of these datasets reduces the racial bias in their judgements. We argue that taboo should not be defined by annotators who are not part of the community, instead the taboos of the community should be defined in relation to its norms.


%\subsection{Bias in Annotators}
%\textcolor{green}{In their work \cite{binns2017like}, the authors demonstrate how different demographics perceive offense differently. With female annotators finding comments less toxic than their male counterparts. Similarly, the authors of \cite{waseem2016you} show that there is disagreement between the perception of amateur and expert annotators, in what they consider hate speech. Most datasets \cite{founta2018large}\cite{davidson2017automated}, used to train offense classifiers do not take the demographics of the annotators into account. This leads to biased training data that propagate throughout the classifier pipeline and lead to classifiers that are biased against languages of certain communities. 

%}
%\subsection{Bias in Training Data} 
%\textcolor{green}{Another source of bias in the classifier pipeline can be attributed to imbalanced training data. In \cite{bolukbasi2016man}, the authors show that language models built word embeddings built on non-representative datasets end up gender bias that reflect social stereotypes. \cite{kennedy2020contextualizing} in their work show that models Hate speech classifiers trained on imbalanced datasets struggle to determine if group identifiers like `gay' or `black' are used in offensive or prejudiced ways. Subsequently they propose regularization techniques to minimize this bias (should remove this line and add to introduction)
%}
%\subsection{Bias in classifiers}
%\textcolor{green}{These datasets can end up propagating their biases to even the state of the art offense detection classifiers like Google’s Perspective.\cite{reichert2020reading} argue that Google’s model tends is more likely to associate higher toxicity scores to comments with identity markers like `woman’ and `gay’, because these identity markers are more frequently referenced in a negative manner in the training data.
%}
%\subsection{Effects of Bias}
%\textcolor{green}{Similarly, \cite{kim2020intersectional} also shows that bias in offense classifiers predominantly affects vulnerable and minority communities. They conclude that African-American tweets were more likely to be labeled as abusive than their white counterparts. 
%}
%\subsection{Racial Bias in Taboo Speech Classifiers}
%\textcolor{green}{The rise in the use of Taboo speech classifiers has seen a rise in works that attempt to quantify, and mitigate, the bias in these classifiers. However, most of these works have focused on bias against identity mentions (e.g. Woman, muslim, queer)\cite{waseem-hovy-2016-hateful}\cite{dixon2018measuring}\cite{park2017one}.


%There is an extremely limited body of work that has dealt with bias against minority communities with shared cultural norms, and in almost all the cases these works have exclusively focused on bias against the African American community.


%Davidson et al. examined racial bias in 5 different twitter datasets annotated for hate speech and abusive language\cite{davidson2019racial}. They compared the predictions of classifiers, trained on these datasets. They found evidence of bias in all the datasets and concluded that tweets belonging to the African American community were significantly more likely to be labeled as hateful or abusive, as compared to those written in mainstream standard American English.


%In the same vein, Sap et al. investigated how annotator insensitivity to difference in dialects can lead to racial bias in hate speech detectors \cite{sap2019risk}. They discovered that self identified African American English tweets were 2 times as likely to be labeld as toxic as compared to those from the mainstream language.

 
%Kim et al. \cite{kim2020intersectional} expanded on this idea of bias against racial communities by investigating the intersectional bias against race and gender. The authors used the Fountana et al. dataset\cite{founta2018large} to show that while African American tweets were 3.7 times more likely to be labeled as abusive, those belonging to African American males were 77\% more likely to be labeled as hateful.
 
 
%The main limitation of all these works has been their focus on a single community. None of the above mentioned works have explored the existence of bias against other cultural communities. Our work goes beyond this. By focusing on a diverse set of 5 cultural communities, it aims to fill in the gaps left by the prior literature.
%}
%\subsection{Works that deal with Community Language Models}
%\textcolor{green}{Another novelty of our work is the use of language models to represent community norms. Language models like BERT\cite{devlin-etal-2019-bert} have been extended to model different languages, with the Multilingual variant of BERT\cite{libovicky2019language} being able to model 104 languages. However, language models are not as commonly used to model dialects and community specific languages.


%Recently, in their work Groenwold et al. \cite{groenwold2020investigating} made use of GPT-2 to model African American Vernacular English (AAVE). Comparing the AAVE model with a Standard American English (SAE) model, they found AAVE and are more likely to have a negative sentiment label than the SAE text. \textbf{this summary is not consistent with the abstract}

%To the best of our knowledge, ours is the one of the first works that takes the knowledge of community language models beyond African American and includes other community languages. Furthermore, our work is the first to use language models to represent community norms and use them to investigate bias in toxic speech classifiers.

%}

%\subsection{Our Novelty}
%\begin{itemize}
%    \item Other works have considered bias in classification
%    \item they have not looked at community `norms'
%\end{itemize}

==> arxiv-acl2022-Suum Cuique_ Studying bias in taboo detection with a community perspective/trash.tex <==
\subsection{Offense depends on Context}
\begin{enumerate}
    \item African-American Language Use: Ideaology and so-called Obscenity
    \item Characterizing Variation in Toxic Language by Social Context
\end{enumerate}
\subsection{Bias in Training Labels}
\subsection{Bias in Classifiers}
\subsection{Empirical Analysis of Multi-Task Learning for Reducing Identity Bias in Toxic Comment Detection}
\subsubsection{Aim}
The paper aims to co-train an LSTM based model to learn both identities and toxicity in comments. The system is then used to predict the toxicity of comments
\subsubsection{How is it related}
This is, in spirit, similar to our work, because we also try to learn the identity of the group by using a language model.
\subsubsection{Where is the bias coming from}
The paper compares the performance of their systems with classifiers that use logistic regression, CNNs etc. They do not compare their classifier with Perspective. The bias that they are are trying to mitigate comes directly from the training data.
\subsubsection{Where is the Data coming from}
They make use of 1,804,874 comments that were part of a Kaggle Dataset provided by Jigsaw (The group behind Google Perspective).
\subsubsection{Groups}
homosexual, black, muslim,jewish, white, average (Note: We are not using White and average language models)
\subsubsection{How are they evaluating their performance}
They use the following three metrics to evaluate their system 
\begin{itemize}
    \item Subgroup AUC: A low AUC score, calculated for a subgroup, is bad
    \item Background Positive, Subgroup Negative AUC (BPSN): Non-toxic comments from the test set with identity and the control are used to get the ROC-AUC. A high ROC-AUC means that a low False Positive Rate.
    \item Generalized Mean of Bias AUC:The AUCs of all subgroups are averaged. A low AUC would indicate that the system is biased towards a particular identity.
\end{itemize}
\subsection{Reading Between the Demographic Lines Reducing Scores of Bias in Toxicity Classifier}
\subsubsection{Aim}
Construct toxicity classifiers to mitigate the effects of unintended bias.
\subsubsection{How is it related}
Along with generating language models for each identity group, they also use a definition of toxicity that is similar to ours. Any comment that has a toxicity score $>0.5$ is assigned a positive label. However, unlike our work they use a two-layer BiDirectional LSTM that predicts a toxicity label. 
\subsubsection{Where is the Data coming from}
They make use of 84,502 tweets from the House of representatives. The identities they are interested in are Political leanings. They also had a set of 405,130 tweets with active identity markers (mentions). Their work in effect compares the bias introduced when you mention your identity vs when you don't. 
\subsubsection{Where is the bias coming from}
At the end of their paper they compare their work with Perspective
\subsubsection{Groups}
Any identity marker.
\subsubsection{How are they evaluating their performance}
AUC, FPR, Comparison with Perspective
\subsection{Contextualizing Hate Speech Classifiers with Post-hoc Explanation}

Bias caused by: Imbalanced datasets
Aim: Use fine-tuned BERT to detect bias towards identity terms.

Manually identify 25 group identifies like Jews, Women.
They extract SOC post-hoc explanations
The dataset used was Gab Hate Corpus and Stormfront corpus. vs NYTimes articles.

The baseline is unregularized BERT and BERT with Word Removal
The authors regularize BERT, they call it BERT+SOC (Sampling and Occlusion)
SOC estimates model agnostic context independent post-hoc feature importance (see: Jin et al. 2020)

\subsection{Intersectional Bias in Hate Speech and Abusive Language Dataset}:

They wanted to investigate whether the human-annotated data used to train hate speech algorithms is biased. More specifically they wanted to analyze whether race and gender generated a biased distribution of hateful and abusive labels.

They used the annotated twitter dataset(Founta et al). The dataset is considered the gold standard.
The dataset did not contain information about race, party identification or gender. 
They did not classify the actual race/gender/political leaning, instead the objective was to classify whether the language features expressed in a tweet were closer to the ones commonly expressed by one racial/gender/partisan group than the other. This is similar to how we are framing our problem.

Their conclusions were that african american tweets were more likely to be labeled as abusive than white tweets, and among the african americans, male tweets were more likely to be classified as hateful compared to the other groups.
African American females were only slightly more likely to be labeled as hateful than their white counterparts.

So in summary - in effect, they had language models and tried to classify the origin of the tweet, by comparing the language.



\subsection{Generating Biased Dataset for Neural Natural Language Processing}

The authors consider cases where datasets are compromised by annotator bias. They propose a neural bias annotator, a generative model that learns to emulate a biased annotator. It is a domain and label agnostic approach, it generates objectively biased samples that explicitly associate features to label. The synthesized samples are claimed to be sufficiently natural and convincing. They aim to make the extent of bias controllable and quantifiable.

The proposed approach is called Conditionally Adversarially Regularized Autoencoder (CARA). CARA is trained to learn a label agnostic latent space where a semantic component - like gender or race, can be added to the latent vectors. This addition acts like a bias trigger signature. 

They find that BERT, RoBERTa ad XLNET trained on the biased dataset can be swayed to classify text samples as the bias target class whenever the target is present.


\subsection{Developing an Online hate classifier for muliple social media platforms.}

The authors collect a total of 197,566 comments from Youtube (ICWSM-18),wikipedia(KAGGLE-18), reddit(ALMEREKHI-19) and twitter(DAVIDSON-17). They compare how well different features and algorithms perforom for hate detection on multiple social media platforms. What were the most impactful features when predicting hate. And how well does a machine learning model learn linguistic characteristics of hate.

They use Simple stylistic features like number of words, number of uppercase, etc, BOW, BERT and word2vec, LIWC. Besides the cross-platform nature, and the analysis the paper is relatively straight forward.

\subsection{Characterizing Variation in Toxic Language by Social Context}
They look at 6.7K potentially toxic tweets from users with different relationship types. Their main hypothesis is that the notion of toxicity depends on the context, the relationship.
The four relationships they looked at were.
there is no connection, there's a symmetric connection, there is a one sided connection.

Using Twitter Streaming API, they tracked 56 terms from HateBase, collecting over 178K messages, for each tweet they collected the tweet's author and recipient, and the relationship between the author and the recipient.

For each tweet, they got a snapshot of it after 2 months. Determining the number of likes retweets and deletion status. 

The had students annotate the tweets. They found messages are more likely to be toxic if there is no relationship between the author and the recipient. And least likely to be toxic if both users know each other. They also used deletions as a proxy variable. While they do not actually talk much about the deletion norms on twitter. I think they have implicitly relied on the idea that deletions are caused by people reporting a tweet. Similar to the annotated sample, they found that tweets are less likely to be deleted if they are sent between people who know each other. And most likely to be deleted if the two users do not know each other.

This paper supports our hypothesis that toxicity/hate is context dependent.

==> casestudy.tex <==
\section{Case Study}
As a case study, we gather a portion of moderated comments from subreddits which are part of one of the communities we tested. 
% 
Since these comments are moderated, we should expect the community language models to give lower scores to these comments, as moderators should be acting as \textit{taboo} language removers\footnote{Note: \textit{taboo} language is not the only reason comments may be moderated on a subreddit.}. 
%
For each subreddit, we check the membership scores for the community of which it belongs. That is, the data of r/LatinoPeopleTwitter is checked against the Hispanic community language model. 
%
We compare the average language model score on the test set used for verifying (section \ref{sect:verification}), against the average of the moderated comments of a subreddit. These results can be found in table \ref{tab:casestudy}.


\begin{table*}[]
    \centering
    \begin{tabular}{c|c|c|c}
         Subreddit & Community & Moderated Text Average & Community Text Average  \\\hline
         LatinoPeopleTwitter & \multirow{2}{*}{Hispanic} & 66.9 & \multirow{2}{*}{78.9} \\
         asklatinamerica &  & 77.0 &\\\hline
         ABCDesis & South Asian & 82.4 & 78.4 \\\hline
         Hawaii & Hawaii & 58.7 & 77.8 \\\hline
         NativeAmerican & \multirow{2}{*}{Native American} & 85.1 & \multirow{2}{*}{71.8} \\
         IndianCountry && 66.8 & \\\hline
         blacklivesmatter & African American & 42.0 & 80.7 \\\hline
    \end{tabular}
    \caption{Comparison of average language models scores of comments composed of moderated comments from a subreddit with the community test sets in section \ref{sect:verification}. Each subreddit's moderated comments are scored with the community language model to which it belongs. }
    \label{tab:casestudy}
\end{table*}


\noindent \textbf{Community Language Models give Lower Scores to Moderated Comments.} We observe that across communities, the community language models score the moderated text lower than the community's test set. 
%
For example, for African American, the average community test score is 80.7 compared to a score of 42.7 for the moderated comments from the subreddit r/blacklivesmatter. 
%
One exception is South Asian, which could indicate that their moderation standards are not easily agreed upon by that community. 


==> graveyard.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{images/LM Distribution Vs NativeAmerican.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distribution Vs. Hispanic.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distributions Vs. Hawaii.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distributions Vs. SouthAsian.pdf}
    \includegraphics[width=0.5\columnwidth]{images/LM Distributions Vs. AfricanAmerican.pdf}
    \caption{Distribution of probabilities from language models against their corresponding test set.}
    \label{fig:NALM}
\end{figure}


\section{Outline}
\begin{enumerate}
\item Model construction

Methods: Two methods: BERT and XLNet.
justify these.

Datasets: reddit collections - justify.



\item Model verification

expect to see probability for native group to be high than for other groups.

\begin{enumerate}
    \item 
    native test set
    
    \item
    Blodgett demographic dataset
    
    \item
    userlevelrace dataset
    
    
\end{enumerate}

\item
exploring bias 

\begin{enumerate}
    \item 
    in classifiers
    
    \item
    in datasets
    \begin{itemize}
        \item Reddit moderated data
        \item Offenseval
        \item other1
        \item other2
    \end{itemize}
    
\end{enumerate}



(must check for consistency with what others find



\end{enumerate}

%
%\subsubsection{Datasets} \label{sect:validDatasets}
%In addition to running validation tests with the held out Reddit data (see Table\ref{tab:LMTestSet}) we use two more datasets for validation.
%These are both Twitter subsets as opposed to Reddit.
%validate our language models by using three datasets.

%We verify our models on three datasets:
%\begin{itemize}
%    \item Demographic16-AA: A dataset by Blodgett et al., which contains demographic-aware topic models for AAE (African American English), White, and Other.
%    The dataset includes a HI set, however, the paper itself does not use this data due to ``uncertainty'' of what the HI model learned. Therefore, we exclude this from our validation process as well. dialects.
%This race-annotated dataset of over 56M tweets has been regarded as the gold standard of AAE language in several papers \cite{sap2019risk, davidson2019racial, groenwold2020investigating, xia2020demoting}.
%The AAE community is comparable to the African American community in our experiments. To make the models more comparable, we sample 50k AAE tweets. Using our language models, we assign alignment scores using each community model to these tweets. 
%\item UserLevelRace-AA: A dataset by Preotiuc-Pietro et al., that contains the self-reported race of Twitter users and their tweets \cite{preotiuc-pietro-ungar-2018-user}. Like with Demographic16, we sample 50k African American tweets to form our third validation dataset. 
%\end{itemize}
%
%The dataset was built using geo-located tweets matched with Census demographic data. They then use a topic modeling approach to estimate the likelihood of each race for a tweet.  
%Their validation test show that non-HI black language tweets show language properties consistent with prior research AAE language.
%The authors estimate the dialect of each tweet by using a demographic aware topic model which leverages race and ethnicity data from the census as well as geocoordinates from the user's twitter profile. 
%
%As we are relying on models trained on Reddit data to predict language belonging to communities formed on Twitter, we expect that our models would experience a degradation in their predictive powers.
%This is because norms vary across social media, even for culturally similar communities. We still expect the norms of the language to dominate over the differences in styles across social media, resulting in our African American model outperforming the other community language models.
%Note that since our models are trained on Reddit data it is possible that estimates are lower for the same community when we use the two Twitter subsets.
%This is because the language model is likely to be shaped by the nuances of that social media platform. However, we expect community norms of language to dominate over differences in styles across social media.
%\vspace{-0.5em}
%\textcolor{red}{Note: The following idea is weak!}
%Even though these datasets are extracted from different social media platforms, our notion of community platform independent. Instead we are grouping subcultures/subreddits\textcolor{red}{NOTE: Not sure which one to go with} into communities based on their shared cultural heritage and norms. 
%A language model trained on a particular platform will learn the nuances of that medium, and is expected to suffer a degradation when tested on the language of another medium. However overall, it would still be able to use the community specific signals to detect the relevant community. And on average, it will outperform the models trained on the other communities.
%\subsection{Validation results}
%We observe the membership score distribution for each community language model on its respective held out Reddit set in 


%\textcolor{green}{The reason for this cutoff is two-fold. First, a cutoff of 0.85 ensures each community language model assigns membership to > 50\% of the language in their respective test sets. Second, this is a stronger number than \cite{blodgett-etal-2016-demographic}, which set a cutoff of 0.8. }


%
%From our observations, we choose a confidence cutoff of 0.85 when deciding whether language belongs to a community. 
%

%\textcolor{green}{As noted in model construction (section \ref{}), BlackPeopleTwitter is a highly popular Reddit community which encourages diversity in its members. This popularity can also cause those who interact with its post to fluctuate}[NOTE: We aren't running experiments to support any claims about the membership makeup of a community]. \textcolor{green}{ This led us to include it in its own model. }


%\textcolor{red}{As noted in model construction (section \ref{}), the popularity of BlackPeopleTwitter on reddit encourages diversity in its membership. This lack of homogeneity means that BlackPeopleTwitter is a community that is distinct from the other African American communities. }

%[NOTE: I HAVE SOME ISSUES/QUESTIONS. I Will engage with BPT after those have been resolved.]
%
%The distribution of memberships scores seems to reinforce this idea of diversity and fluctuation in the BlackPeopleTwitter community. 
%
%A highly diverse/fluctuating community, would not settle on common language, thereby making it difficult for a language model to learn language for that community.
%
%Because of these observations, we do not include BlackPeopleTwitter scores in the main analysis discussions going forward. 
%\par\textcolor{green}{We also test each community language model on the test sets for the other models to ensure that our models are not assigning high membership scores to all languages. These results can be found in table \ref{tab:LMTestSet}.}

==> trash.tex <==
\subsection{Offense depends on Context}
\begin{enumerate}
    \item African-American Language Use: Ideaology and so-called Obscenity
    \item Characterizing Variation in Toxic Language by Social Context
\end{enumerate}
\subsection{Bias in Training Labels}
\subsection{Bias in Classifiers}
\subsection{Empirical Analysis of Multi-Task Learning for Reducing Identity Bias in Toxic Comment Detection}
\subsubsection{Aim}
The paper aims to co-train an LSTM based model to learn both identities and toxicity in comments. The system is then used to predict the toxicity of comments
\subsubsection{How is it related}
This is, in spirit, similar to our work, because we also try to learn the identity of the group by using a language model.
\subsubsection{Where is the bias coming from}
The paper compares the performance of their systems with classifiers that use logistic regression, CNNs etc. They do not compare their classifier with Perspective. The bias that they are are trying to mitigate comes directly from the training data.
\subsubsection{Where is the Data coming from}
They make use of 1,804,874 comments that were part of a Kaggle Dataset provided by Jigsaw (The group behind Google Perspective).
\subsubsection{Groups}
homosexual, black, muslim,jewish, white, average (Note: We are not using White and average language models)
\subsubsection{How are they evaluating their performance}
They use the following three metrics to evaluate their system 
\begin{itemize}
    \item Subgroup AUC: A low AUC score, calculated for a subgroup, is bad
    \item Background Positive, Subgroup Negative AUC (BPSN): Non-toxic comments from the test set with identity and the control are used to get the ROC-AUC. A high ROC-AUC means that a low False Positive Rate.
    \item Generalized Mean of Bias AUC:The AUCs of all subgroups are averaged. A low AUC would indicate that the system is biased towards a particular identity.
\end{itemize}
\subsection{Reading Between the Demographic Lines Reducing Scores of Bias in Toxicity Classifier}
\subsubsection{Aim}
Construct toxicity classifiers to mitigate the effects of unintended bias.
\subsubsection{How is it related}
Along with generating language models for each identity group, they also use a definition of toxicity that is similar to ours. Any comment that has a toxicity score $>0.5$ is assigned a positive label. However, unlike our work they use a two-layer BiDirectional LSTM that predicts a toxicity label. 
\subsubsection{Where is the Data coming from}
They make use of 84,502 tweets from the House of representatives. The identities they are interested in are Political leanings. They also had a set of 405,130 tweets with active identity markers (mentions). Their work in effect compares the bias introduced when you mention your identity vs when you don't. 
\subsubsection{Where is the bias coming from}
At the end of their paper they compare their work with Perspective
\subsubsection{Groups}
Any identity marker.
\subsubsection{How are they evaluating their performance}
AUC, FPR, Comparison with Perspective
\subsection{Contextualizing Hate Speech Classifiers with Post-hoc Explanation}

Bias caused by: Imbalanced datasets
Aim: Use fine-tuned BERT to detect bias towards identity terms.

Manually identify 25 group identifies like Jews, Women.
They extract SOC post-hoc explanations
The dataset used was Gab Hate Corpus and Stormfront corpus. vs NYTimes articles.

The baseline is unregularized BERT and BERT with Word Removal
The authors regularize BERT, they call it BERT+SOC (Sampling and Occlusion)
SOC estimates model agnostic context independent post-hoc feature importance (see: Jin et al. 2020)

\subsection{Intersectional Bias in Hate Speech and Abusive Language Dataset}:

They wanted to investigate whether the human-annotated data used to train hate speech algorithms is biased. More specifically they wanted to analyze whether race and gender generated a biased distribution of hateful and abusive labels.

They used the annotated twitter dataset(Founta et al). The dataset is considered the gold standard.
The dataset did not contain information about race, party identification or gender. 
They did not classify the actual race/gender/political leaning, instead the objective was to classify whether the language features expressed in a tweet were closer to the ones commonly expressed by one racial/gender/partisan group than the other. This is similar to how we are framing our problem.

Their conclusions were that african american tweets were more likely to be labeled as abusive than white tweets, and among the african americans, male tweets were more likely to be classified as hateful compared to the other groups.
African American females were only slightly more likely to be labeled as hateful than their white counterparts.

So in summary - in effect, they had language models and tried to classify the origin of the tweet, by comparing the language.



\subsection{Generating Biased Dataset for Neural Natural Language Processing}

The authors consider cases where datasets are compromised by annotator bias. They propose a neural bias annotator, a generative model that learns to emulate a biased annotator. It is a domain and label agnostic approach, it generates objectively biased samples that explicitly associate features to label. The synthesized samples are claimed to be sufficiently natural and convincing. They aim to make the extent of bias controllable and quantifiable.

The proposed approach is called Conditionally Adversarially Regularized Autoencoder (CARA). CARA is trained to learn a label agnostic latent space where a semantic component - like gender or race, can be added to the latent vectors. This addition acts like a bias trigger signature. 

They find that BERT, RoBERTa ad XLNET trained on the biased dataset can be swayed to classify text samples as the bias target class whenever the target is present.


\subsection{Developing an Online hate classifier for muliple social media platforms.}

The authors collect a total of 197,566 comments from Youtube (ICWSM-18),wikipedia(KAGGLE-18), reddit(ALMEREKHI-19) and twitter(DAVIDSON-17). They compare how well different features and algorithms perforom for hate detection on multiple social media platforms. What were the most impactful features when predicting hate. And how well does a machine learning model learn linguistic characteristics of hate.

They use Simple stylistic features like number of words, number of uppercase, etc, BOW, BERT and word2vec, LIWC. Besides the cross-platform nature, and the analysis the paper is relatively straight forward.

\subsection{Characterizing Variation in Toxic Language by Social Context}
They look at 6.7K potentially toxic tweets from users with different relationship types. Their main hypothesis is that the notion of toxicity depends on the context, the relationship.
The four relationships they looked at were.
there is no connection, there's a symmetric connection, there is a one sided connection.

Using Twitter Streaming API, they tracked 56 terms from HateBase, collecting over 178K messages, for each tweet they collected the tweet's author and recipient, and the relationship between the author and the recipient.

For each tweet, they got a snapshot of it after 2 months. Determining the number of likes retweets and deletion status. 

The had students annotate the tweets. They found messages are more likely to be toxic if there is no relationship between the author and the recipient. And least likely to be toxic if both users know each other. They also used deletions as a proxy variable. While they do not actually talk much about the deletion norms on twitter. I think they have implicitly relied on the idea that deletions are caused by people reporting a tweet. Similar to the annotated sample, they found that tweets are less likely to be deleted if they are sent between people who know each other. And most likely to be deleted if the two users do not know each other.

This paper supports our hypothesis that toxicity/hate is context dependent.
